Generative Temporal Models with Memory

We consider the general problem of modeling temporal data with long-range dependencies, wherein new observations are fully or partially predictable based on temporally-distant, past observations. A sufficiently powerful temporal model should separate predictable elements of the sequence from unpredictable elements, express uncertainty about those unpredictable elements, and rapidly identify novel elements that may help to predict the future. To create such models, we introduce Generative Temporal Models augmented with external memory systems. They are developed within the variational inference framework, which provides both a practical training methodology and methods to gain insight into the models' operation. We show, on a range of problems with sparse, long-term temporal dependencies, that these models store information from early in a sequence, and reuse this stored information efficiently. This allows them to perform substantially better than existing models based on well-known recurrent neural networks, like LSTMs.

==> OnModifiedKLDivergence.tex <==
% \section{On KL divergence between prior and corrective posterior distributions}
% \label{appdx:modifiedKL}

% Starting with the KL divergence between two $K$ dimensional multivariate Gaussians $q$ and $p$ with full covariance matrices $\Sigma_q$ and $\Sigma_p$ and means $\mu_q$ and $\mu_p$:
% \begin{equation}
% \text{KL}(q || p) = \frac{1}{2}\left[\text{log } \frac{\text{det}(\Sigma_p)}{\text{det}(\Sigma_q)} - K + \text{tr}(\Sigma_p^{-1}\Sigma_q) + (\mu_q-\mu_p)^T\Sigma_p^{-1}(\mu_q-\mu_p)\right]
% \end{equation} 
% Assuming diagonal covariance matrices, we can derive:
% \begin{equation}
% \text{KL}(q || p) = \frac{1}{2}\left[\text{log } \frac{\prod^K_{i=1}(\Sigma_p)_{i,i}}{\prod^K_{i=1}(\Sigma_q)_{i,i}} - K + \sum^K_{i=1}\frac{(\Sigma_q)_{i,i}}{(\Sigma_p)_{i,i}} + (\mu_q-\mu_p)^T\Sigma_p^{-1}(\mu_q-\mu_p)\right]
% \end{equation} 
% \begin{equation}
% \text{KL}(q || p) = \frac{1}{2}\left[\sum^K_{i=1} \text{log }\frac{(\Sigma_p)_{i,i}}{(\Sigma_q)_{i,i}} - K + \sum^K_{i=1}\frac{(\Sigma_q)_{i,i}}{(\Sigma_p)_{i,i}} + \sum^K_{i=1}\frac{(\mu_q-\mu_p)_{i}^2}{(\Sigma_p)_{i,i}}\right]
% \end{equation} 
% \begin{equation}
% \text{KL}(q || p) = \frac{1}{2}\sum^K_{i=1}\left[ \text{log }\frac{(\Sigma_p)_{i,i}}{(\Sigma_q)_{i,i}} - 1 +\frac{(\Sigma_q)_{i,i}}{(\Sigma_p)_{i,i}} + \frac{(\mu_q-\mu_p)_{i}^2}{(\Sigma_p)_{i,i}}\right]
% \end{equation} 

% Given $\forall i \in \{1,.., K\}$,
% \begin{equation}
% (\mu_p)_{i} = \Theta_z^\mu(\vPsi_t)_i
% \end{equation} 
% \begin{equation}
% (\Sigma_p)_{i,i} = \Theta_z^\sigma(\vPsi_t)_i
% \end{equation} 
% \begin{equation}
% (\mu_q)_{i} = \Phi_z^\mu(\vPsi_t, \vx_t)_i=\Theta_z^\mu(\vPsi_t)_i+\Delta^\mu(\vPsi_t, \vx_t)_i
% \end{equation} 
% \begin{equation}
% (\Sigma_q)_{i,i} = \Phi_z^\sigma(\vPsi_t, \vx_t)_i=\Theta_z^\sigma(\vPsi_t)_i\cdot\Delta^\sigma(\vPsi_t, \vx_t)_i
% \end{equation} 
% \begin{equation}
% (\mu_q - \mu_p)^2_{i} = ((\mu_q)_{i} - (\mu_p)_{i})^2 = \Delta^\mu(\vPsi_t, \vx_t)^2_i
% \end{equation} 
% \begin{equation}
% (\Sigma_q)_{i,i}/(\Sigma_p)_{i,i} = \Delta^\sigma(\vPsi_t, \vx_t)_i
% \end{equation} 
% \begin{equation}
% \end{equation} 

% Then, the KL divergence becomes:
% \begin{equation}
% \text{KL}(q_{\phi} || p_\theta)= \frac{1}{2}\sum^K_{i=1}\left[-\text{log }\Delta^\sigma(\vPsi_t, \vx_t)_i - 1 +\Delta^\sigma(\vPsi_t, \vx_t)_i + \frac{\Delta^\mu(\vPsi_t, \vx_t)^2_i}{\Theta_z^\sigma(\vPsi_t)_i}\right]
% \end{equation} 

%
%
%
%\begin{equation}
%\text{KL}(q_{\phi} || p_\theta) = \frac{1}{2} \left[  -\text{log}\left(     
%|\Delta^\sigma(\vPsi_t, \vx_t)| \right) - K + \text{Tr}\left(
%\Delta^\sigma(\vPsi_t, \vx_t) \right) +\frac{\Delta^\mu(\vPsi_t, \vx_t)^2}{\Theta_z^\sigma(\vPsi_t)}\right]
%\end{equation}

==> OnStepwiseVarBound.tex <==
\section{Sequential Latent Variable Models and Variational Inference}
\todo{Mevlana: I can move it to an appendix once we are happy.}

A natural extension of latent variable models like VAEs to modeling sequential data $\{\mathbf{x}_1, \mathbf{x}_2..., \mathbf{x}_T\}$ can be defined by introducing latent variables at each time-step and modeling the joint probability of $\{\mathbf{x}_{\le T}, \mathbf{z}_{\le T}\} = \{\mathbf{x}_1, \mathbf{x}_2..., \mathbf{x}_T, \mathbf{z}_1, \mathbf{z}_2..., \mathbf{z}_T\}$, which can be factorized as:
\begin{equation}
p_\theta(\mathbf{x}_{\le T}, \mathbf{z}_{\le T}) = \prod_{t=1}^T p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t})
\end{equation}

We wish to maximize the joint likelihood of data $p_\theta(\mathbf{x}_{\le T})$. Applying the variational principle, the objective function now becomes a step-wise variational lower bound through a number of steps:

\begin{equation}
\text{log }p_\theta(\mathbf{x}_{\le T}) \ge \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})} \left[\text{log } p_\theta(\mathbf{x}_{\le T}, \mathbf{z}_{\le T})- \text{log } q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})\right]
\end{equation}

\begin{equation}
\text{log }p_\theta(\mathbf{x}_{\le T}) \ge \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})} \left[\text{log } \prod_{t=1}^T p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t}) p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})
- \text{log } \prod_{t=1}^T q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le T}) \right]
\end{equation}
Since $q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T}) = \prod_{t=1}^T q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le T})$ does not factorize further into a step-wise product, we make use of the \emph{filtering} assumption (or choice) $q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le T}) = q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le t})$ on the approximate posterior and move the products out of the logarithms:
\begin{equation}
 \ge \E_{\prod_{t=1}^T q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le t})} \left[ \sum_{t=1}^T \text{log }p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t}) + \text{log } p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})
- \text{log } q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le t})\right]
\end{equation} 

\begin{equation}
 \ge \E_{\prod_{t=1}^T q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le t})}
 \left[\sum^T_{t=1}  \text{log } p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t})-\text{KL}(q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_{\le t})||p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})) \right]\text{WRONG}
\end{equation}

We can make mild assumptions about the dependency structure, namely, $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t}) = p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})$ and $p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t}) = p_\theta(\mathbf{x}_t| \mathbf{z}_t)$ and therefore the joint distributions is:
\begin{equation}
p_\theta(\mathbf{x}_{\le T}, \mathbf{z}_{\le T}) = \prod_{t=1}^T p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})p_\theta(\mathbf{x}_t| \mathbf{z}_t)
\end{equation}
where $p_\theta(\mathbf{z}_1|\mathbf{z}_{<1}) = p_\theta(\mathbf{z}_1)$. This enforces the temporal relationships within the sequences to be modeled only among the latent variables through the joint prior $p_\theta(\mathbf{z}_{\le T})$.

In this factorization, the prior distribution at each time step $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})$ is now conditional only on the latent variables from previous time steps and the \emph{observation model} $p_\theta(\mathbf{x}_t| \mathbf{z}_t)$ is again a highly non-linear function of only the current step's latent variables similar to VAEs.

The variational bound now becomes:
\begin{equation}
\text{log }p_\theta(\mathbf{x}_{\le T}) \ge \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})} \left[\sum^T_{t=1} \text{log } p_\theta(\mathbf{x}_t| \mathbf{z}_t)+ \text{log } p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}) - \text{log } q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)\right]
\end{equation}
\begin{equation}
 \text{log }p_\theta(\mathbf{x}_{\le T}) \ge \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})}\left[\sum^T_{t=1} \text{log } p_\theta(\mathbf{x}_t| \mathbf{z}_t) -\text{KL}(q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)||p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})) \right]\text{WRONG}
\end{equation}

As in the standard VAEs, we learn the \emph{generative model} and the \emph{recognition model} jointly by maximizing this variational lower bound with respect to their parameters where the samples from the \emph{recognition model} $\mathbf{z}_1, \mathbf{z}_2..., \mathbf{z}_t \sim q_\phi(\mathbf{z}_{\le t}|\mathbf{x}_{\le t})$ are created forward in time (i.e. filtering) by sampling from $q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)$ at each time step [($q_\phi(\mathbf{z}_{t}|\mathbf{z}_{<t}, \mathbf{x}_{\le t})$ in the more general case]. 



==> VIbackground.tex <==
\subsection{Variational Inference}
\label{subsect:GM}
A generative model specifies a joint probability $p(\vx, \vz)$ over observable variables $\vx$ and latent variables $\vz$. Maximum likelihood learning in a generative model requires marginalisation of the latent variables, which is typically an intractable operation to compute. 
To sidestep this problem, we make use of variational inference \citep{jordan1999introduction} [cite], which transforms the difficult integration over the latent space into an optimisation problem. 
The goal of learning is to maximise the marginal log-likelihood $\log p_\theta(\vx) = \int p_\theta(\vx, \vz) d \vz$. For any distribution $q_\phi(\vz | \vx)$ \todo{Mevlana: this version is much clearer I believe}, we note the following identity
\begin{align}
\text{KL}[q_\phi(\vz | \vx) || p_\theta(\vz | \vx)] & = \E_{q_\phi(\vz | \vx)} \log \frac{q_\phi(\vz | \vx)}{p_\theta(\vz | \vx)} \nonumber \\
% & = \E_{q_\phi(\vz | \vx)} \log \frac{q_\phi(\vz | \vx) p_\theta(\vx)}{p_\theta(\vz | \vx) p_\theta(\vx)} \nonumber \\
& = \E_{q_\phi(\vz | \vx)} \log \frac{q_\phi(\vz | \vx) p_\theta(\vx)}{p_\theta(\vx, \vz)} \nonumber \\
& = \log p_\theta(\vx) - \E_{q_\phi(\vz | \vx)} \log \frac{p_\theta(\vx, \vz)}{q_\phi(\vz | \vx)} 
\end{align}
The quantity $-\E_{q_\phi(\vz|\vx)|} \log \frac{p_\theta(\vx, \vz)}{q_\phi(\vz|\vx)}$ is abbreviated $\mathcal{F}$, and is called the \emph{variational free energy}. 
A lower bound to the marginal log-likelihood is constructed by observing that $\log p_\theta(\vx) = \text{KL}[q_\phi(\vz) || p_\theta(\vz | \vx)] + \mathcal{F} \geq \mathcal{F}$ since the Kullback-Leibler divergence is non-negative. 

Instead of maximising the marginal log-likelihood directly, variational methods maximise the variational free energy $\mathcal{F}$ with respect to both $p$ and $q$. By learning the variational parameters $\phi$ of $q$, the cost of inference is amortised \citep{rezende2014stochastic}. The variational distribution $q$ approximates the posterior $p(\vz | \vx)$ and is known as a \emph{recognition} or \emph{inference} model.

The expectations in the variational free energy are typically unknown, and the gradients of the free energy are computed by Monte Carlo estimators, using pathwise derivative estimators (reparameterisation trick) for continuous latent variables \citep{rezende2014stochastic, kingma2014stochastic}. The resulting combination of latent variable models, trained by amortised variational inference with Monte Carlo gradient estimates, is commonly referred to as a variational auto-encoder (VAE).

% \todo{Mevlana: We should be mentioning amortized inference here.}
\todo{outline: \\
background on generative modeling (why generative models) \\
background on temporal models \\
background on memory systems \\
background on variational methods for time series models \\
breaking calculations into maps: prior map $h_{t-1} \to z_t$; posterior map $(h_{t-1}, x_t) \to z_t$; observation map $(z_t, h_{t-1}) \to x_t$; transition map $(h_{t-1}, z_t, x_t) \to h_t$ \\
adding memory into maps; types of memory \\
note: difficulty of optimising lstm-like models; solutions not only rarely generalise to test but also do not even find solutions on training. \\
}

==> experiments.tex <==
\section{Experimental Tasks}
\label{sect:experimentalTasks}
\todo{greg: switch this to past tense; fill out intuitions for tasks}
We tested our models on seven tasks that probed their capacity to learn and make predictions about temporal data with complex dependencies. Tasks involved image-sequence modeling, and offered tests of deduction, spatial reasoning, and one-shot generalisation. Example training sequences are provided for each task described below. For tasks with artificial data sets, pseudo-code to generate training sequences is provided in Appendix \ref{pseudocodeForTasks}.

\subsection{Perfect Recall}
\begin{figure}[h!]
	\centering
    \includegraphics[width=\linewidth]{figures/PerRecallExample}
    \caption{Example sequence for the \emph{perfect recall} task using a pre-recall interval $l=20$ followed by a recall interval $k=5$.}
    \label{fig:perfectRecallExample}
\end{figure}
Training sequences consisted of $k$ randomly sampled MNIST digits to be remembered during a pre-recall interval, which extended for $l$ time steps. Thus, $l-k$ digits were distractor stimuli. A recall interval occurred after $l$ steps, during which the first $k$ images were presented again. We constructed variants of the task with $k=5$ and $l \in \{20, 25, 55\}$. Figure \ref{fig:perfectRecallExample} shows a typical training sequence for this task. To succeed at this task, the models must encode and store the first $k$ images, protect them during the distractor interval, and retrieve them during the recall interval. Successful use of memory would elicit a drop in the KL-divergence during the recall interval, since information stored in memory -- and not information extracted from the current observation -- would be used for image reconstruction.

% The observations at every point in time are images from the MNIST data set. The sequence consists of $l$ random images, followed by a sequence of $k$ images copied from the first $k$ digits of the initial $l$-length sequence. In the example, the random interval $l = 20$ and the recall interval $k=5$. In order to learn such sequences, the models must have the ability to learn dependencies with temporal delays of length $l$. We seek temporal models that are able to solve this task for various settings of $l$, and when asked to generate data, should generate sequences with exactly this pattern.
\subsection{Parity Recall}
\begin{figure}[h!]
	\centering
    \includegraphics[width=\linewidth]{figures/ParRecallExample}
    \caption{In the \emph{parity recall} task, the recall interval consisted of images indicating the evenness or oddness of each of the initial $k$ images.}
    \label{fig:parityRecallExample}
\end{figure}
In contrast to the previous experiment, in which exact recall of the images was demanded, in the parity recall task we asked the model to identify and report on a latent property of the data. During the recall interval, the model must generate a sequence of $k$ $0$-s and $1$-s, matched to the parity of the first $k$ images. That is, the first recalled digit should be a zero if the first digit in the initial sequence was odd, and one if it was even. Figure \ref{fig:parityRecallExample} shows a typical training sequence. Successful models, then, need to implicitly classify input digits. Although the \textit{computation} required for this task is more complicated than for perfect recall, the information content that is to be stored is actually smaller; i.e. a single bit per image. \adam{Started changing tense up to this point -- will wait until final edits to continue this process}

%The temporal structure of the sequences in this task is fixed in the same manner as the sequences in the \emph{Perfect Recall} task. Again, in each training sequence, we first pick a random sequence of digits for $l$ time steps. Instead of replicating the instances from this \emph{random interval} in the \emph{recall interval} however, we take an arbitrary function over the MNIST classes, in this case, \emph{evenness-oddness} of digits, and apply it to the first $k$ instances to obtain their parity. Then, the last $k$ instances are picked based on the parity of the first $k$ instances where \emph{evenness} is represented by a uniformly random instance of digit $1$ and \emph{oddness} is represented by a uniformly random instance of digit $0$. An example training sequence can be seen in Figure \ref{fig:parityRecallExample}, where the first $5$ digits' parity determines the samples at the last $5$ time steps. In this task, the last $k$ samples are a much more complicated function of the past compared to the first task, but the information content to carry over is much smaller (i.e. a single bit of information). The models have to implicitly learn to separate digits into two sets according to their parity and simply carry this knowledge across time to learn the temporal relationship.
% This task builds on the difficulty of the perfect recall task by demanding that the network not just recall information to which it was previously exposed, but rather, demanding that it learn a more complicated function relating to the classes of digits contained the $k$ samples at the beginning of the sequence. Specifically, the network must output a random sample of the digit 1 if the corresponding sample in $k$ is even, and must output a random sample of the digit 0 if the corresponding sample in $k$ is odd. Thus, the network must implicitly learn an odd-even digit classifier for the samples contained in $k$. 

\subsection{One-Shot Recall}
\begin{figure}[h!]
	\centering
    \includegraphics[width=\linewidth]{figures/OneShotRecallExample}
    \caption{For the \emph{one-shot recall} task, sequences at test time are created from a set of characters that were not used during training. Even so, perfect recall should still be possible.}
    \label{fig:OmniRecallExample}
\end{figure}
We also examine the abilities of the GTMMs to memorise novel information by testing on sequences of data on which they have not been directly trained. A typical training sequence is shown in Figure \ref{fig:OmniRecallExample}, where the images at every point in time are drawn from the Omniglot data set \citep{lake2015human}. The training data consist of all 50 alphabets with three characters excluded from each alphabet. The unseen characters are used to form new, unseen sequences at test time. The task is otherwise the same as the perfect recall task, but the demands on the generative model and memory are more substantial.  
%
%A model's ability to robustly handle context that it was not trained on is also an important quality to evaluate, especially with respect to the preservation of information across long time-scales. In this task, we extend the \emph{Perfect Recall} task to the one-shot learning case in order to determine whether the learned recall ability applies to data that is not seen during training. 
%Again, in each training sequence, we first pick a random sequence of instances for $l$ time steps, but this time from a subset of Omniglot Characters Dataset \cite{omniglot} instead of MNIST. Similar to the Perfect Recall task, the last $k$ instances are replicated from the first $k$ instances from the \emph{random interval}. The subset of characters used for training sequences is created by excluding $3$ characters from each alphabet in Omniglot. 
%In addition these training sequences, we also create short sequences of length $k$ called \emph{unseen context sequences} which consist only of random instances from the held out characters of each alphabet in Omniglot. 
%During the evaluation of the models for their ability to do one-shot recall on unseen data, we present these \emph{unseen context sequences} at the first $k$ steps to condition on and generate the rest of the sequence from the model. If the model is able to apply the recall ability to novel data that was not encountered during training, then it would be able to replicate these \emph{unseen context sequences} at the end of the generated sequence instead of a random sample sequence. The Figure \ref{fig:OmniRecallExample} displays a training sequence picked from the Omniglot dataset that uses only the subset of characters that are assigned to training.

\subsection{Learning Dynamic Dependencies}
\begin{figure}[h!]
	\centering
    \includegraphics[width=\linewidth]{figures/DynDepExample}
    \caption{Training sequence for the \emph{dynamic dependency} task following an index-and-recall game in which each image digit provides a positional reference to the next digit in the sequence order.}
    \label{fig:dynDepExample}
\end{figure}
The preceding tasks have all demanded ordered recall of the sequence.
Here, we test whether recall in a more complicated order is possible.
A typical training sequence is shown in Figure \ref{fig:dynDepExample}. We begin with a sequence of $l$ digits as before. 
The next $k$ digits are generated by an ``index-and-recall'' game. 
In the figure example, the final digit in the pre-recall interval is an 8.
The numerical value of the digit indicates from which position in the sequence the next digit is copied. Here, position 8 contains a 3, which is the first digit in the recall interval. Position 3 contains a 0, and so on. Successful models must therefore learn to classify digits and to use the class labels to find images based on their temporal order of presentation.
%In the two tasks presented above, dependencies are fixed between specific time steps, namely the first and last $k$ time steps, even if they are long-range dependencies. In this task however, we wish to evaluate our models' ability to cope with data sequences that have dynamic temporal dependencies. 
%To accomplish this, we exploit the labels of MNIST digits as a form of 'address in time' while creating the training sequences. First, a \emph{random sequence} of length $l$ is created as before. In each step $t$ of the next $k$ picks, we determine the digit label of the most recently picked instance, $L_{t-1}$, and use this number as an 'address in time' over the \emph{random interval} and replicate the instance from the $L_{t-1}$th time step.
%For example, in the example training sequence presented in Figure \ref{fig:dynDepExample}, the digit $3$ at the beginning of the \emph{recall interval} is a replica of the digit instance from the eighth time step on the \emph{random interval} because the instance that comes just before the recall interval is an $8$. Similarly, the digit $0$ that comes after the digit $3$ is a replica of the instance from the third time step from the \emph{random interval} etc. Therefore, the dependency structure of the last $k$ steps are dynamically determined based on the context of what has been picked in the previous step. In this task, the models have to implicitly learn to a classifier of digits without supervision and use this information to look back in time and attend to the right content from the past to correctly learn the temporal relationship and be able to generate similar sequences that have such complicated temporal structures.
% In this task, we wish to show that our GTMs are able to determine where to direct its attention in the time sequence based on the context of what it has generated already while generating the next step. We want to show that our GTMs can implicitly learn to bind a higher level concept of what it generates to actual time steps and learn data sequences that have non-stationary time delays.
\subsection{Similarity-Cued Recall}
\begin{figure}[h!]
	\centering
    \includegraphics[width=\linewidth]{figures/ConRecallExample}
    \caption{Example training sequence for the \emph{similarity-cued recall} Task.}
    \label{fig:contentDepExample}
\end{figure}
The last task probes positional indexing, but here we construct a task that demands content-based addressing.
In each training sequence, we first present a \emph{random sequence} of digits for $l$ time steps. The $k$ digits in the \emph{recall interval} are a randomly chosen, contiguous sub-sequence of length $k$ from the pre-recall interval (Figure \ref{fig:contentDepExample}).
To solve this task, a model must be able to use the first image in the recall interval as a cue, find the most similar image to the cue that it has seen previously, and produce the temporal sequence that followed it.

\subsection{Navigation in an MNIST Map}
\begin{figure}[h!]
	\centering
    \includegraphics[height=5cm]{new_figures/MnistMaze/MnistMazeField}
    \caption{A random walk action sequence is provided to the model along with images found at each location. At boundaries, the action sequence is restricted to stay in bounds. Each action is provided as a conditioning variable for generation that is not modeled itself.}
    \label{fig:mnist_maze}
\end{figure}
An important motivation for developing GTMMs is the desire to improve the capacity of agents to understand the spatial structure of their environments. 
As an example problem, we create a 2D environment represented by a $4 \times 4$ grid, where each grid cell contains a random MNIST digit (Figure \ref{fig:mnist_maze}). 
In this case, instead of an agent, we take a random walk on the grid using actions up, down, left, and right for 25 steps to move between neighbouring locations, receiving an observation corresponding to the current grid cell. The actions are always treated as context variables and are not predicted by the GTMMs.
We expect that the GTMMs conditioned on random walk action sequences will be able to generate the same observation in case a grid cell is revisited in an action sequence; that is, the GTMM should maintain a coherent map of an environment.

%\break
\subsection{Towards Coherent Generation in Realistic 3D Environments}
\todo{pump up but manage expectations a bit about what has been achieved}
\begin{figure}[h!]
	\centering
    \includegraphics[width=\linewidth]{new_figures/Rot/rot15}
    \caption{A training sequence for a 30 timestep in-place rotation, where the period until repetition is approximately 15 steps.}
    \label{fig:Rot15Example}
\end{figure}
Ultimately, we wish to design agents that operate in realistic environments and can learn from sequential information, using memory to form predictions. 
These agents should possess spatiotemporally coherent memories of environments, understanding that walls typically do not shift and that undisturbing movements change camera angles but not scene arrangements. 
Our first study of this problem is to test whether GTMMs can maintain consistent predictions when provided with frames from an in-place rotation of a camera for two full turns.
Our experiments take place in a procedurally-generated 3D maze environment with random wall configurations, textures, and object positions.

The rotational dynamics of the environment include acceleration, so each frame does not represent a view from an angle that is equally distributed around the unit circle. The models must cope with this structure. 
Additionally, because the frames are captured at discrete moments, the models must learn to interpolate past views after the full turn, instead of merely copying frames from the first rotation.
The rotational period is $t=15$ steps, and a full episode takes $t=30$ steps.
An example training sequence is shown in Figure \ref{fig:Rot15Example}.
A successful generative model of this data must create random environment panoramas and generate views consistent with the panorama on the second full turn.

==> nips_version/conclusion.tex <==
\section{Conclusion}
In this paper, we introduce the \emph{Introspection Network}, an \emph{internal} attention mechanism over the latent variables, as a building block of generative and temporal models that can learn from sequential data complex temporal relationships with long-term delays. Our experiments focus on artificial data sequences based on benchmark datasets that exposes the weaknesses of previously proposed models. We show that the introduction of the Introspection Network into our GTMs vastly improves the ability and efficiency of learning the inherent temporal relationships in data and allows our models to generate coherent sample sequences that explains the data as a whole. 

\todo{additional thoughts, 1) unsupervised use of memory systems. 2) stochastic and uncertainty handling that is not done with other memory stems.}

==> nips_version/genModels.tex <==
\section{Variational Generative Temporal Models}
\label{sect:GTM}
Generative temporal models (GTMs) provide powerful tools for assessing the probability of temporal data sequences and for making temporal predictions. Latent variable GTMs, such as Kalman filters, hidden Markov, state-space and changepoint models \citep{sarkka2013bayesian}, are amongst the most popular approaches and model the temporal structure between observed data $\vx_1, \vx_2, \ldots, \vx_T$, using a set of corresponding latent variables $\vz_1, \vz_2, \ldots, \vz_T$ with a Markov dependency. Their joint probability is:
\begin{equation}
p_\theta(\vx_{1:T}, \vz_{1:T}) = \prod_{t=1}^T p_\theta(\vz_t| f_z(\vz_{<t}))p_\theta(\vx_t| f_x(\vz_t)) 
\label{eq:jointprob}
\end{equation}
where $p(\mathbf{z}_1|\mathbf{z}_{<1}) = p(\mathbf{z}_1)$, and denoting any model parameters by $\theta$. The likelihood function $p_\theta(\vx_t| f_x(\vz_t))$ can be any distribution appropriate for the observed data, such as a Gaussian for continuous observations or a Bernoulli distribution for binary data. The conditional probabilities are specified by non-linear functions $f_z$ and $f_x$ represented by deep neural networks for the latent dynamics and the likelihood function, respectively. This non-linear dependency makes these models instances of non-linear dynamical systems or alternatively, as stochastic recurrent neural networks.

Learning in this model requires marginalisation of the latent variables, which is typically intractable. To allow for tractability, we make use of variational inference \citep{jordan1999introduction}, which transforms the difficult integration into an optimisation problem. For GTMs, the application of the variational principle results in an optimisation objective that is a sum of per-step variational free energies:
\begin{equation}
\mathcal{F} = \sum^T_{t=1} \E_{q(z_t|z_{<t})}\left[\text{log } p_\theta(\mathbf{x}_t| \mathbf{z}_t)\right] -\text{KL}[q_\phi(\vz_t|\vz_{<t},\vx_t)||p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})]
\label{eq:FE}
\end{equation}
where a distribution $q(\vz_t| \vz_{<t},\vx_t)$ is introduced to approximate the unknown posterior distribution over the latent variables.
Popular variational approaches represent the approximate posterior distribution as a recognition or inference model $q_\phi(\vz_t| f_q(\vz_{<t},\vx_t))$, whose conditional dependencies are non-linear functions $f_q$ that introduce a set of global variational parameters $\phi$, allowing for amortisation of the cost of inference \citep{rezende2014stochastic}. The expectations in \eqref{eq:FE} are typically unknown, and the gradients of the free energy are computed by Monte Carlo estimators, using pathwise derivative estimators (reparameterisation trick) for continuous latent variables \citep{rezende2014stochastic, kingma2014stochastic}. The resulting combination of latent variable models trained by amortised variational inference that use Monte Carlo gradient estimation is commonly referred to as a variational auto-encoder (VAE); in this paper we develop new temporal VAEs.

A wide family of temporal VAEs can be created by considering different latent transition probability distributions. In variational RNNs \citep{NIPS2008_3567} the transition probability $p(\vz_t | f_z(\vz_{<t}, \vx_{<t}))$ is dependent on \textit{both} past latent variables and past observations, with the dynamics captured with an LSTM network. In principle, such a model is able to model temporal sequences with complex dependency structures, since the LSTM is able to reduce the effects of vanishing gradients and allow for learning across long time periods. An alternative VRNN would consider transition probabilities $p(\vz_t | f_z(\vz_{<t}))$ that depends on past latent variables only, similar to eq. \eqref{eq:jointprob}. A second alternative would use $p(\vz_t | f_z( \vx_{<t}))$ that depends  on the past observations only. Due to their strength as GTMs, these three temporal VAEs form the set of baselines to which we shall compare.

%%\subsection{Sequential Latent Variable Models with Variational Inference}
%VAEs [11, 17] have been shown to be an effective latent variable model for learning complex multimodal distributions over the data space in non-sequential settings, where the joint probability distribution is defined as:
%\begin{equation}
%p_\theta(\mathbf{x}, \mathbf{z}) = p_\theta(\mathbf{x}|\mathbf{z})p_\theta(\mathbf{z})
%\end{equation}
%When the \emph{observation model} $p_\theta(\mathbf{x}|\mathbf{z})$ is parameterized as a highly nonlinear function in this setting, the posterior distribution $p_\theta(\mathbf{z}|\mathbf{x})$ becomes intractable. VAEs introduce a \emph{recognition model} $q_\phi(\mathbf{z}|\mathbf{x})$ as a variational approximation to the posterior using the lower bound:
%\begin{equation}
%\text{log }p_\theta(\mathbf{x}) \ge \E_{q_\phi(\mathbf{z}|\mathbf{x})} [- \text{log } q_\phi(\mathbf{z}|\mathbf{x})+ \text{log } p_\theta(\mathbf{x}, \mathbf{z})]=  -\text{KL}(q_\phi(\mathbf{z}|\mathbf{x})||p_\theta(\mathbf{z}))+\E_{q_\phi(\mathbf{z}|\mathbf{x})}(\text{log }p_\theta(\mathbf{x}|\mathbf{z}))
%\end{equation}
%Typically, $q_\phi(\mathbf{z}|\mathbf{x})$ is parameterized by a deep neural network whose outputs are $\{\boldsymbol{\mu}, \boldsymbol{\sigma^2}\}$ of a diagonal Gaussian $\mathcal{N}(\boldsymbol{\mu}, \text{diag}(\boldsymbol{\sigma}^2))$. The \emph{generative model} $p_\theta(\mathbf{x}, \mathbf{z}) $ and the \emph{recognition model} $q_\phi(\mathbf{z}|\mathbf{x})$ are trained jointly by maximizing the variational lower bound with respect to their parameters, while using the \emph{reparameterization trick}[11]  to obtain low-variance stochastic gradient estimates with respect to the parameters of $q_\phi(\mathbf{z}|\mathbf{x})$.
%
%A natural extension of latent variable models like VAEs to modeling sequential data $\{\mathbf{x}_1, \mathbf{x}_2..., \mathbf{x}_T\}$ can be defined by introducing latent variables at each time-step and modeling the joint probability of $\{\mathbf{x}_1, \mathbf{x}_2..., \mathbf{x}_T, \mathbf{z}_1, \mathbf{z}_2..., \mathbf{z}_T\} : \{\mathbf{x}_{\le T}, \mathbf{z}_{\le T}\}$, which can be factorizes as:
%\begin{equation}
%p_\theta(\mathbf{x}_{\le T}, \mathbf{z}_{\le T}) = \prod_{t=1}^T p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t})
%\end{equation}
%In our model, we make mild assumptions about the dependency structure, namely, $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t}) = p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})$ and $p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t}) = p_\theta(\mathbf{x}_t| \mathbf{z}_t)$ and therefore:
%\begin{equation}
%p_\theta(\mathbf{x}_{\le T}, \mathbf{z}_{\le T}) = \prod_{t=1}^T p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})p_\theta(\mathbf{x}_t| \mathbf{z}_t)
%\end{equation}
%where $p_\theta(\mathbf{z}_1|\mathbf{z}_{<1}) = p_\theta(\mathbf{z}_1)$. This enforces the temporal relationships within the sequences to be modeled only among the latent variables through the prior.
%
%In this factorization, the prior distribution at each time step $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})$ is now conditional on the latent variables from previous time steps and the \emph{observation model} $p_\theta(\mathbf{x}_t| \mathbf{z}_t)$ is again a highly non-linear function of only the current step's latent variables similar to VAEs which require approximate inference of the joint posterior $\prod_{t=1}^T p_\theta(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)$ through the \emph{recognition model} $q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T}) = \prod_{t=1}^T q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)$. The objective function now becomes a step-wise variational lower bound:
%
%\begin{equation}
%\text{log }p_\theta(\mathbf{x}_{\le T}) \ge \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})} \left[- \text{log } q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})+ \text{log } p_\theta(\mathbf{z}_{\le T}, \mathbf{x}_{\le T})\right]
%\end{equation}
%\begin{equation}
%\text{log }p_\theta(\mathbf{x}_{\le T}) \ge \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})} \left[\sum^T_{t=1} - \text{log } q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)+ \text{log } p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}) + \text{log } p_\theta(\mathbf{x}_t| \mathbf{z}_t)\right]
%\end{equation}
%%\begin{equation}
%% \text{log }p_\theta(\mathbf{x}_{\le T}) \ge \sum^T_{t=1} -\text{KL}(q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)||p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})) + \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})}\left[\sum^T_{t=1} \text{log } p_\theta(\mathbf{x}_t| \mathbf{z}_t)\right]
%%\end{equation}
%\begin{equation}
% \text{log }p_\theta(\mathbf{x}_{\le T}) \ge \sum^T_{t=1} -\text{KL}(q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)||p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})) + \E_{q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)}\left[\text{log } p_\theta(\mathbf{x}_t| \mathbf{z}_t)\right]
%\end{equation}
%
%As in the standard VAEs, we learn the \emph{generative model} and the \emph{recognition model} jointly by maximizing this variational lower bound with respect to their parameters where the samples from the \emph{recognition model} $\mathbf{z}_1, \mathbf{z}_2..., \mathbf{z}_t \sim q_\phi(\mathbf{z}_{\le t}|\mathbf{x}_{\le t})$ are created forward in time (i.e. filtering) by sampling from $q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)$ at each time step. 

%
%\subsection{Variational Recurrent Neural Networks}
%In recent work, Bengio et.al proposed using an LSTM to parameterize the distributions $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})$ (Figure 1.c+a), $p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t})$ (Figure 1.c+b) and $q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_{\le t})$
%(Figure 1.c+d) where the recurrent parameters from the LSTM are shared among these distributions. This model does not make the mild assumptions we mentioned earlier and instead feeds the generated/given observations $\mathbf{x}_t$ back into the recurrent network. Therefore, the variational bound this model maximizes is given as:
%%\begin{equation}
%%\sum^T_{t=1} -\text{KL}(q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_{\le t})||p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})) +  \E_{q_\phi(\mathbf{z}_{\le T}|\mathbf{x}_{\le T})}\left[\sum^T_{t=1}\text{log }p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t})\right]
%%\end{equation}
%\begin{equation}
%\sum^T_{t=1} -\text{KL}(q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_{\le t})||p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})) +  \E_{q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_{\le t})}\left[\text{log }p_\theta(\mathbf{x}_t| \mathbf{z}_{\le t}, \mathbf{x}_{<t})\right]
%\end{equation}
%Using an RNN architecture that has special additive interactions that improve gradient flow like LSTM is motivated by highly non-linear nature of the distributions involved in recurrence like $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t}, \mathbf{x}_{<t})$ which would cause the gradients to vanish in regular RNNs in only a few time steps. In principle, a model that uses an additive memory system like LSTM can model temporal relationships over very large time-scales and it has been shown to model delays up to hundreds of time steps in some practical settings. In this work, our results suggest that the effects of interference that decay the gradient only linearly in time (rather than exponentially) in those settings might be much more severe in the stochastic setting of variational approximate inference for generative modeling of data sequences. 
%%\pagebreak
%\begin{figure}[t]
%    \centerline{\includegraphics[width=1\linewidth]{figures/modelWith2}}
%    \label{IntrospectionGraph}
%    \vspace{-0.2cm}
%    \caption{Architecture of the \emph{Introspection Network}.}
%    \vspace{-0.5cm}
%\end{figure}



==> nips_version/intro.tex <==
\section{Introduction}
%
An important aspect of human cognition is the ability to make use of introspective knowledge, in which we make decisions and take actions by re-using previously-formed and internal judgements of our data streams and environments. Our aim is to equip machine learning systems, and deep generative models in particular, with this ability to recall previously-formed beliefs, resulting in introspective generative models that are able to learn faster about their data streams, better establish complex dependencies between events that are temporally distant, and be more flexible in the range of tasks to which they can be applied. The act of introspection implies the use of memory systems to enable the reuse of previously formed beliefs and computation. We therefore develop new introspective probabilistic models of  sequential data that are augmented by an external memory.

Learning deep generative models of temporal sequences that simultaneously allow for simulation of future events, capturing long-range temporal dependencies, maintaining temporal coherence, and are efficient and scalable to large data sets, is a challenging task. Generative temporal models (GTMs) that meet these requirements are essential for tasks in spatial navigation, counterfactual reasoning and simulation-based planning. Most recently developed deep generative models \citep{kingma2014stochastic, rezende2014stochastic, gregor2015draw, eslami2016attend, rezende2016one} are models of i.i.d. data. These static generative models can be applied to an impressive range of problems including image compression, data simulation, image denoising, dimensionality reduction, missing data completion, uncertainty estimation, one-shot generalisation, and semi-supervised classification, all of which stand to be inherited by their temporal extensions. 

Generative temporal models appear in many forms. State-space models are the most widely used and model temporal dynamics using a latent stochastic transition function \citep{sarkka2013bayesian}. Recurrent neural networks learn temporal dynamics using a deterministic transition function over the observed data. A hybrid approach is especially interesting, and uses a generative observation model, such as a latent variable model, Boltzmann machine or Markov random field, combined with temporal dynamics described by a recurrent neural network, such as long short-term memory network (LSTM) \citep{hochreiter1997long} or gated recurrent unit (GRU). Examples of this include recurrent restricted Boltzmann machines \citep{NIPS2008_3567}, LSTM-conditional random field models \citep{huang2015bidirectional} and variational RNNs \citep{chung2015recurrent}. In such models, the ability to generate data and the capacity for long-term dependency tracking are bound together through the recurrent network. These processes can interfere with each other, especially when learning from  high-dimensional visual data with complex temporal dependencies. We separate the generative ability of the model from its ability to track long-term dependencies by designing GTMs that make use of memory and introspection.

The design of models with an external memory is common in machine learning. By an \textit{external memory} we refer to a buffer of fixed capacity into which the results of computation (memories) at different times is stored and then reused at a later stage. In temporal settings we refer to an episodic memory, since memories are stored over a temporal window (or episode), storing memories of recent events only. In statistical machine learning, non-parametric methods, clustering and mixture models \citep{wasserman2006all}, use external memories to store the actual data or sufficient statistics of it (such as projections and cluster centres). In reinforcement learning and robotics, the concept of stigmergy is used, which extends the perception-action feedback loop to include an external memory \citep{peshkin2001learning}. In deep learning, neural Turing machines \citep{graves2014neural} and memory networks \citep{weston2014memory} have been developed as means of overcoming the limitations and widening the applicability of recurrent neural networks.

It is natural then to consider the combination of memory systems with deep generative models. Li et al. \citep{li2016learning} developed a memory-augmented deep generative model for i.i.d data. In that setting, the addition of memory does not allow the model to form richer posterior approximations, leading to limited improvement over standard variational auto-encoders \citep{rezende2014stochastic,kingma2014stochastic}, and where more significant gains can be made by a focus on richer posteriors \citep{gregor2015draw,rezende2016one}. The inclusion of memory in temporal settings has the potential for far greater gains, and is what we develop in this paper. We begin by describing the general approach for designing generative temporal models, and variational inference for such models (section \ref{sect:GTM}), and then make the following contributions:
 \vspace{-2mm}
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item We develop an introspection network, which is a memory system for generative temporal models that combines an episodic memory with attention and gating.
\item We develop new temporal variational autoencoders that effectively separate the ability for dependency tracking and generative ability, allowing for complex dependency structure in temporal data to be discovered.
\item We demonstrate that our model is general enough to discover the hidden temporal structure in five challenging tasks, which range from generative variants of the copy task, to one-shot reasoning across temporally distant time periods.
\item We show in a visual maze environment that our model can learn from actions and observations to form a coherent understanding of its environment, exploiting its memory to efficiently generate under loop-closure. 
\end{itemize}


==> nips_version/introspection.tex <==
\section{Introspective Generative Temporal Models}
%
The GTMs we have described thus far, while highly general, use an LSTM both as a means of capturing temporal dependencies and as a context for reconstruction and generation. This can be problematic since the these two requirements can cause interference, resulting in gradients of one task dominating the other at different points during training and resulting in slower learning. For the experiments that we show in section \ref{sect:exp}, the typical learning dynamics for VRNN-type models is to focus on the reconstruction aspect of the loss function during the first part of training, and only once this is suitably learnt, to model the temporal structure in the data. With such learning dynamics, important parts of the temporal structure can easily be ignored. 

One way to overcome the problem of interference and slow learning is to use an \textit{introspective generative model} to
separate the role of dependency tracking from generation. Our model requires two components: a memory mechanism that allows the model to introspectively reuse latent variables from the past; and modified generative models and inference networks that depend on introspective context. Figure \ref{fig:stochcompgraph} depicts the high-level components of the model and how they are combined.
%
\begin{figure}[t]
	\centering
    \includegraphics[height=0.35\linewidth]{figures/modelVF1.png}
    \includegraphics[height=0.35\linewidth]{figures/modelVF2.png}
    \caption{Stochastic computational graph showing components on an introspective generative model}
    \label{fig:stochcompgraph}
\end{figure}
%
\subsection{Introspection Networks}
An introspection network is a memory mechanism that is responsible for capturing the temporal structure of data. At every time point, an introspection network uses it memory to produce a memory-context $\vPsi_t$, which supplies information about the temporal structure to other parts of the model; all dependencies on the past are routed through this network. An introspection network comprises three components: an \emph{episodic memory} into which we write latent variables $\vz_t$ as they are generated; a \emph{controller}, that uses an LSTM network to direct attention over occupied memory locations, providing the mechanism by which memories are retrieved; and a \emph{gating mechanism} that is used to selectively route memories to the generative model when multiple memories are simultaneously retrieved.

\paragraph{Episodic memory.} The episodic memory $\vM$ is a first-in-first-out buffer with at most $L$ storage location into which we insert, or write, latent variables $\vz_t$ as they are generated at each temporal step. It is natural to store the latent variables in memory, since they provide the compressed representation of the data at each time point. But it is also possible to store other quantities, such as deterministic transformations of the latent variables as done by \citep{li2016learning}. 

\paragraph{Control mechanism.} The control mechanism is responsible for retrieval from the episodic memory, and achieves this by using an LSTM to track temporal relationships and provides the context for the soft attention that is used. At every time step $t$, the controller first updates the hidden states and output of its LSTM network $f_{rec}$, which fuses information from the previous hidden state $\vh_t$ and the previously generated latent variable $\vz_{t-1}$. If additional side information $\vc_{t}$ is available, then this can be included as an input. The sole responsibility of this LSTM is temporal dependency tracking. In the most general setting, $R$ memories can be retrieved simultaneously, which requires the use of multiple `read-heads'. Each read-head implements a soft attention using weights $\vw^r_t$, which are produced at every step using an attention network $f_{att}$ and the output of the LSTM $\vh_t$. Finally, the content of the memory $\vM_{t-1}$ is read as a weighted sum for each read-head, producing the retrieved-memory $\vpsi^r_t$. 
\begin{eqnarray}
\textrm{State update} & \vh_t = f_{rec}(\vh_{t-1}, \vz_{t-1}, \vc_{t}) & \\
\textrm{Attention} & \vw^{r}_t = f_{att}(\vh_{t}); \quad \|\vw^{r}_t\|=1 & \\
\textrm{Retrieved memory} & \vphi^r_t = \vw^r_t \cdot \vM_{t-1} & 
\end{eqnarray}
When the memory buffer is not full, the function $f_{att}$ adjusts the length of its output according to the number of stored memories and normalizes each weight vector accordingly. A number of attention functions $f_{att}$ can be used, including: softmax $\mathbf{w}_{t} = e^{k(\mathbf{h}_{t})}/\sum e^{k(\mathbf{h}_{t})}$, normalized linear $\mathbf{w}_{t} = {k(\mathbf{h}_{t})}/\sum {k(\mathbf{h}_{t})}$ or Gaussian attention $\mathbf{w}_{t} = \mathcal{N}(i|\mu'(\mathbf{h}_{t}),\sigma'(\mathbf{h}_{t}))$; the functions $k, \mu', \sigma'$ are deep networks. The controller is not sensitive to this choice, hence we present results using softmax attention only.

\paragraph{Gating mechanism.} The ability to retrieve multiple memories $\vphi_t^r$ simultaneously makes it possible for the latent variables $\vz_{t}$ to depend on a varying number of latent variables from the past. To facilitate this, a gating mechanism is used to maintain or attenuate the retrieved memories. A parameter vector $\vg_t^r$ is learnt for each retrieved memory and is passed through a sigmoid function $\sigma(\cdot)$, producing a gate for the retrieved memories for each read-head $r$. 
\begin{eqnarray}
\textrm{Memory-context} & \vPsi_t^r = \vphi_t^r \odot \sigma(\vg^r_{t-1}) & 
\end{eqnarray}
The final memory context $\vPsi_t$ is the concatenation of the memory-contexts for each read-head $\vPsi_t = [\vPsi_t^1, \vPsi_t^2, \ldots, \vPsi_t^R]$, and forms the introspective context that is passed to the generative model for inference and prediction. The complete flow of information in the introspection network is shown in the stochastic computational graph in figure \ref{fig:stochcompgraph}.

\subsection{Modified Generative and Inference Models}
The introspection network removes all responsibility for dependency tracking from the generative and inference models used in temporal VAEs. As a result, the generative model \eqref{eq:jointprob} and inference need only be adapted to make use of the memory-context $\vPsi_t$, which  involves modifying them to condition on this context.

\paragraph{Conditional generative model.} We explore two types of prior distribution for the latent variables $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})$. The simpler case uses a $K$-dimensional latent variable with a diagonal Gaussian distribution. A more powerful alternative uses an auto-regressive Gaussian distribution, which generates a $K$-dimensional latent variable using an autoregressive chain of $D$ $k$-dimensional Gaussian distributions (giving $K= kD$).
\begin{eqnarray}
\textrm{Diagonal } & p_\theta(\vz_t| \vz_{<t}) = \mathcal{N}(\vz_t |f_\mu(\vPsi_t), f_\sigma(\vPsi_t)) & \\
\textrm{Auto-regressive } & p_\theta(\vz_t| \vz_{<t}) = \prod_{d=1}^D p_\theta(\mathbf{z}^d_t| \mathbf{z}_{<t}, \vz_t^{<d}) = \prod_{d=1}^D \mathcal{N}(\vz_t^d |f_\mu(\vPsi_t, \vz^{<d}_t), f_\sigma(\vPsi_t, \vz^{<d}_t)) &
\label{eq:introspPrior}
\end{eqnarray}
The mean and variance of the Gaussian distribution is obtained using non-linear functions $f_\mu$ and $f_\sigma$ that depend on the memory context $\vPsi_t$ obtained at each time point. There is no direct dependency between the latent variables at successive time points, since all dependency is through $\vPsi_t$ and the introspection network. The likelihood function $p(\vx_t | f_x(\vz_t))$ remains unchanged from that used in \eqref{eq:jointprob}. This generative specification is that of a deep latent Gaussian model \citep{rezende2014stochastic}, but it is easy to extend this to more complex models such as those used in DRAW \citep{gregor2015draw}, AIR \citep{eslami2016attend}, and other sequential generative models \citep{rezende2016one}. Figure \ref{fig:stochcompgraph} shows a stochastic computational graph for this generative process.

\paragraph{Conditional inference model.} We also specify the approximate posterior distribution as a Gaussian distribution that is dependent on the memory context $\vPsi_t$. We design the inference model to have a mean that shares parameters with the prior through the function $f_\mu(\vPsi_t)$, with an additional term $\Delta_\mu(\vPsi_t, \vx_t)$ that corrects the prior belief based on the observed data. We use a similar parameterisation for the variance with a variance correction term  $\Delta_\sigma(\vPsi_t, \vx_t)$. 
\begin{equation}
 q_{\phi}(\vz_t|\vz_{<t},\vx_t) = \mathcal{N}(\vz_t |f_\mu(\vPsi_t)+\Delta_\mu(\vx_t, \vPsi_t), f_\sigma(\vPsi_t)\cdot \Delta_\sigma(\vx_t, \vPsi_t) )
\end{equation}
The closed-form solution for the KL divergence becomes (and is derived in the appendix):
\begin{equation}
\text{KL}(q_{\phi} || p_\theta) = \frac{1}{2} \left[  -\text{log}\left(     
|\Delta_\sigma(\mathbf{x}_t, \vPsi_t)|    \right) - D + \text{Tr}\left(
\Delta_\sigma(\mathbf{x}_t, \vPsi_t) \right) +\frac{\Delta_\mu(\mathbf{x}_t, \vPsi_t)^2}{\sigma(\vPsi_t)}\right]
\end{equation}
The parameterization based on correction terms has advantages for optimization: the KL divergence does not depend on the prior function $f_{\mu}(\vPsi_t)$ and allows for easier optimisation of this function; gradients that are propagated to the prior, come not only from the KL divergence term, but also from the stochastic gradients backpropagated from the latent variables. \todo{need help explaining this} 

A forward pass of an introspective GTM involves, at each time step: using the introspection network to provide a memory-context; using this context as part of the inference of the observed data to produce a sample of the latent variable; using this sample and the generative model to reconstruct the observed data point. The training algorithm is a simple modification of the standard algorithm for variational autoencoders \cite{kingma2014stochastic, rezende2014stochastic}, with two additional steps for reading a memory-context at each point, and writing generated samples to the memory buffer. This model is scalable and has complexity of $O(NJD^2)$ for $N$ data points and $J$ layers with an average size of $D$-dimensions, which matches that for other deep generative models and large scale classification systems. The additional complexity added by the instrospection system is $O(LK)$ for $L$ memory slots and $K$-dimensional latent variables. %\todo{should an algo be added?} 
%The algorithm is summarised in algorithm \ref{alg:introspVAE}. 


% MEVLANA HELP WITH TIHIS
%\begin{algorithm}[h!]
%\caption{VAE with Normalizing Flow}
%\begin{algorithmic}
%\STATE{Parameters: $\vphi $ variational, $\vtheta$ generative}
%\WHILE{not converged}
%    \STATE{$\vx \leftarrow $} \COMMENT{Get mini-batch}
%    \STATE{$\vz_0 \sim q(\bullet | \vx)$}
%    \STATE{$\vz_K \leftarrow f_{K} \circ f_{K-1} \circ   \ldots   \circ  f_{1} ( \vz_0 )$}
%    \STATE{$\J(\vx) \approx \J(\vx,\vz_K)$}
%        \STATE{$\Delta \vtheta \propto -\nabla_{\theta} \J(\vx)$}
%        \STATE{$\Delta \vphi \propto -\nabla_{\phi} \J(\vx)$}
%\ENDWHILE
%\end{algorithmic}
%\label{alg:introspVAE}
%\end{algorithm}

%\begin{algorithm}[t!]
%\caption{Training Introspective GTMs}
%\label{alg:introspVAE}
%\end{algorithm}


% In this section, we introduce the \emph{Introspection Network}, an episodic memory and soft attention mechanism over the latent variables of a generative and temporal model (GTM). With \emph{Introspection Network} based GTMs, we are interested in efficiently modeling data sequences where there are high levels of time-inhomogeneity, high levels of sparsity in the dependency structure and finite but very long time-scale relationships. However, we also wish to retain the ability to model data that has highly time-homogeneous and densely connected dependency structures for time-scales where this is efficient for additive memory based GTMs like VRNNs (and variants).
%
%The main goal of the \emph{Introspection Network} is to provide an efficient mechanism for modeling the distributions $p_\theta(\mathbf{z}_t| \mathbf{z}_{<t})$ and $q_\phi(\mathbf{z}_t|\mathbf{z}_{<t},\mathbf{x}_t)$, which are the temporal aspects of the GTM in our setting. Next, we will detail the architecture that parameterizes of both of these distributions:

%The generative model produces its latent variables $\mathbf{z}_{t}$ by first \emph{introspectively} processing the past to read the subset of latent variables to condition on. At every time step, the \emph{control mechanism} updates its hidden state and output, denoted $h$, using the recurrence equation:
%\begin{equation}
%\mathbf{h}_t = f_{rec}(\mathbf{h}_{t-1}, \mathbf{z}_{t-1}), \hspace{25pt} \mathbf{h}_t = f_{rec}(\mathbf{h}_{t-1}, \mathbf{z}_{t-1}, \mathbf{c}_t)\text{[Conditional]}
%\end{equation}
%where $f_{rec}$ is a recurrent neural network like LSTM.

%The output of the RNN is then fed into the function $f_{att}$ that outputs the weights of soft-attention for each read head. Next, the contents of memory stored in $\mathbf{M}_{t-1}$ are retrieved as a weighted sum for each read head. 
%\begin{equation}
%\mathbf{w}^{r}_t = f_{att}(\mathbf{h}_{t}), \hspace{25pt} \|\mathbf{w}^{r}_t\|=1: \forall r\in \{1,...,R\}
%\end{equation}
%\begin{equation}
%\boldsymbol{\varphi}^r_t = \mathbf{w}^r_t \cdot \mathbf{M}_t
%\end{equation}
%At each time step, the latent variable $\mathbf{z}_{t}$ can depend on a different number of variables from the past. 


==> nips_version/results.tex <==
\section{Experimental Results}
\label{sect:exp}
\begin{figure}[t]
    \includegraphics[width=1\linewidth]{figures/generators6}
	\vspace{-0.5cm}
    \caption{Artificially generated training sequences for different tasks based on MNIST/Omniglot datasets and sequences from videos of bouncing balls in a box. In the first four tasks, samples from the last $k$ time steps have inherent dependencies to the samples from the beginning of sequences. At top, we provide the time indices or 'addresses' that are relevant for the Context-Addressed Dependency Task. In this task, the sample at the last step is identical to the $5$th sample (white box) in the sequence because the previous sample (red box) was an instance of digit $5$. The same relationship exists in all of the last $k$ steps.}
	\vspace{-0.5cm}
    \label{generators}
\end{figure}
\subsection{Evaluation Methodology}
We evaluate the \emph{Introspection Network} based GTMs (\emph{IN}-GTM) by comparing them against VRNNs \cite{chung2015recurrent} described in section \ref{sect:GTM} on five tasks that expose different aspects of temporal modelling  that a GTM should satisfy. For each task, we created temporal sequences based on benchmark datasets, e.g., MNIST\cite{MnistCitation}, Omniglot\cite{omniglotCitation} and Bouncing Balls in a Box\cite{NIPS2008_3567}. A successful GTM should perform well in all tasks and generate compelling samples that mimic the temporal relationships embedded in the sequences. These tasks are:
\begin{description}[leftmargin=*,topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item[Perfect Recall Task.] Tests the ability to preserve information without interference across long time-scales efficiently.
\item[Even-Odd Transition Task.] Tests the ability to learn arbitrary and complex relationships between time steps.
\item[Context-Addressed Dependency Task] tests the ability to condition on specific places in the time sequence based on the context of what has been generated already while generating the next step.
\item[One-Shot Recall Task.] Tests the ability to do one-shot generalisation, i.e. successfully apply learned temporal relationships to examples that are never seen during training.
\item[Stochastic Bouncing Balls Task.] Tests the ability to model the stationary distribution of the sequences where there are inherent multimodalities involved.
\end{description} 
%
% in their temporal relationships and train our GTMs to discover these relationships from training sequences.
%If the models are able to learn the underlying distributions of the sequences properly, they should be able to generate sample sequences that mimic the sequences from training.

%\subsubsection{Learning}
We train each model with stochastic gradient descent on the variational lower bounds \eqref{eq:FE} using the Adam optimizer [12], with a learning rate of 0.001. We experimented with different latent variable sizes $K=\{10, 20, 50\}$ and used a minibatch size of $10$ for \emph{IN}-GTMs and $10$ or $24$ for VRNN variants. For both \emph{IN}-GTMs and VRNNs, the functions that parameterize the inference and the generative models are $3$-layer convolutional and deconvolutional residual networks \cite{he2015deep}, respectively. In addition, we experimented with much higher capacity networks for VRNNs with larger MLPs and LSTM hidden units (we discuss the relevant two cases $h=200$ and $h=300$ in our results) compared to \emph{IN}-GTMs. In \emph{IN}-GTMs, we always use an episodic memory of maximum size equal to the length of the training sequences minus one. This length can be in the order of hundreds (see Appendix \ref{AppendResults} for results with $100$ step sequences) without a heavy memory burden as long as the latent space is compact. In comparison, in the small number of experiments where VRNN variants had some success modeling temporal relationships of length $<15$, they had to use more memory overall than \emph{IN}-GTMs that was successful at modeling relationships of length $>50$ .

Initialization of the attention mechanism however is an important factor during optimization since, as the memory size increases, there is a linearly increasing interference in the temporal signal which reduces the signal-to-noise ratio. In the \emph{Introspection Network} architecture, we allocate \emph{parallel} read heads that are initialized with biases that allow for \emph{local} search of the specific parts of the episodic memory in order to increase temporal exploration and speed up optimization. For a temporal sequence of $100$ steps, having $5$ \emph{parallel} heads which have relatively high biases for sub-sequences $[1, 20], [21, 40], [41, 60], [61, 80], [81, 100]$ respectively, can speed up learning tremendously compared to initializing all biases uniformly. During our experiments, we have seen that even with a sharp initialization of these biases, the read heads eventually move to locations with low initial biases during training if they have to in order to model the temporal relationships.\todo{make this fit into text}

\subsection{Tasks and Results}
% 
\begin{description}[style=unboxed, leftmargin=0cm]
\item [Perfect Recall Task] In this task, the training sequences consist of MNIST digits. In each training sequence, we first create a \emph{random sequence} of digits for $l$ time steps. Then, for $k$ time steps, we repeat the same samples from the beginning of the \emph{random sequence} we created earlier, which results in length $L=l+k$ sequences. In the first row of Figure \ref{generators}, we show an example training sequence with $k=5$ where the samples from the last $5$ time steps are the same as the samples from the first $5$ time steps. In order to learn such sequences, the models must to have the ability to learn signals with temporal delays of length $l$. 

\item [\normalfont \emph{Results and comparison}:] In Figure \ref{Task1}, we present samples from an \emph{IN}-GTM that was trained on such sequences of length $L = 50$ (see Appendix \ref{AppendResults} for $L = 100$). We observe that the last $k=5$ steps were generated based on the past generations through perfect recall by focusing on the relevant parts of the sequence with the attention mechanism (see attention weights at top of Figure \ref{Task1}). 

In Figure \ref{ResKLVRNN}(left), we compare \emph{IN}-GTMs against VRNN variants in this task by displaying the evolution of the KL divergence term for the last recall step during training. This term is proportional to the number of bits of information required to reconstruct the sample at that step using the previous samples. If the temporal relationship is learned and the model can do a perfect recall using the past, this value would be very low ($<5$ nats) compared to the number of bits required for a random MNIST digit ($~20$ nats). 

We observe that for \emph{IN}-GTMs, the KL divergences go to $~3$ nats (accomplishes perfect recall) in $<10$k training iterations in a stable way when the temporal delays for recall are around $L = 50$ and $L = 100$ time steps. On the other hand, we present results from VRNN variants only for $L = \{3, 5, 10\}$ sequences. Throughout our experiments, these models were \textbf{not} able to learn the perfect recall relationship with temporal delays of length $>10$. Even in the case of $L = \{5, 10\}$, majority of our experiments did not succeed and there was a large variation in the number of steps of training it took for these models to learn the temporal relationship, whereas \emph{IN}-GTMs have been robust throughout. E.g. one of the two successful models for $L = 3$ in Figure \ref{ResKLVRNN} learns in $<10$k iterations while the other takes $>100$k iterations. 

We believe here is an exponential growth of 




\begin{figure}[t]
%    \includegraphics[height=0.5\linewidth]{figures/KLDivergences}
%    \includegraphics[width=0.4\linewidth]{figures/VrnnSamples}
%    \centerline{\includegraphics[trim={0 0 0 12.cm},clip, width=1.016\linewidth]{figures/Task7/50/AttentionLastStep}}
%    \includegraphics[trim={0 13.2cm 0 0},clip, width=\linewidth]{figures/Task1/50/sample}
%    \includegraphics[width=\linewidth]{figures/Task3/sample4}
%    \includegraphics[width=\linewidth]{figures/Task12/50/sample2}
%    \includegraphics[width=\linewidth]{figures/Task7/50/sample4}

\begin{subfigure}{\textwidth}
  \centering
	\includegraphics[width=1\linewidth]{figures/VRNNComparison}
   \caption{Left: KL divergences for \emph{Introspection Network} based GTMs (\emph{IN}-GTM) and VRNNs during training with sequences from \textbf{Perfect Recall Task} with various lengths. Right: Sample sequences generated by VRNNs in the same task.}
	\label{ResKLVRNN}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
%	\centerline{\includegraphics[trim={0 0 0 12.cm},clip, width=1.016\linewidth]		{figures/Task7/50/AttentionLastStep}}
	\centerline{\includegraphics[trim={0 2cm 0 0},clip, width=1.016\linewidth]		{figures/hinton50}}
	\includegraphics[trim={0 13.2cm 0 0},clip, width=\linewidth]{figures/Task1/50/sample}
  \caption{Bottom: Corresponding samples from \emph{IN}-GTM trained on sequences from \textbf{Perfect Recall Task} with $l = 45$ and $k = 5$. Top: Distribution of attention weights from the \emph{Introspection Network} when sampling the last step of the sequence.}
	\label{Task1}
\end{subfigure}%

\begin{subfigure}{\textwidth}
  \centering
    \includegraphics[width=\linewidth]{figures/Task3/sample4}
  \caption{Samples from \emph{IN}-GTM trained on sequences from \textbf{Even-Odd Transition Task} with $l = 45$ and $k = 5$.}
  	\label{Task2}
\end{subfigure}

\begin{subfigure}{\textwidth}
  \centering
    \includegraphics[width=\linewidth]{figures/Task12/50/sample3}
  \caption{Samples from \emph{IN}-GTM trained on sequences from \textbf{Context-Addressed Dependency Task} with $l = 45$ and $k = 5$.}
   \label{Task3}
\end{subfigure}

\begin{subfigure}{\textwidth}
  \centering
    \includegraphics[width=\linewidth]{figures/Task7/50/sample4}
  \caption{Samples from \emph{IN}-GTM trained on sequences from \textbf{One-Shot Recall Task} with $l = 45$ and $k = 5$. This \emph{IN}-GTM uses an auto-regressive latent space with 2 levels of depth.}
  \label{Task4}
\end{subfigure}

\caption{Results for \emph{Introspection Network} based GTMs (\emph{IN}-GTM) and VRNNs. In all the figures with samples, the rows represent different sample sequences and columns represent the time steps.}
\end{figure}

\item [\textbf{Even-Odd Transition Task}] The temporal structure of the sequences in this task mimics the previous task.
%, i.e. last $k$ samples are related to the first $k$ samples from the beginning of the \emph{random sequence}.
Instead of repeating past samples however, we take an arbitrary function over the MNIST classes, \emph{evenness-oddness} of digits, and apply it to samples from the past to obtain their parity. Then, the last $k$ samples are generated based on the parity of the first $k$ samples from the \emph{random sequence} where even is represented by random digit $1$ and odd is represented by random digit $0$ as can be seen in the second row of Figure \ref{generators}. In this task, the last $k$ samples are a much more complicated function of the past compared to the first task and the models have to implicitly learn a classifier of the digits to learn the temporal relationship well.

\item [\normalfont \emph{Results}:] In Figure \ref{Task2}, we display samples generated by the \emph{IN}-GTM model after training it with sequences of length $50$. We see that the model generates random $0$s and $1$s in the last five steps based on the parity of the first five samples in the sequence (Refer to appendix for class transition matrices between the first and last five steps of the sequences and the full algorithm for the generative process for this task).

%Similar to the first task, we first create a \emph{random sequence} of MNIST digits for $l$ time steps. In this task, instead of repeating past samples for the next $k$ time steps, we take an arbitrary function over the MNIST classes (evenness/oddness) of the samples from the past and generate random $1$s and $0$s corresponding to evenness of the first $k$ samples from the beginning of the \emph{random sequence}. In the first row of figure \ref{generators}, we show an example sequence for $k=5$ where the samples from the last $5$ time steps are the same as the samples from the first $5$ time steps


%. In the first row of figure \ref{generators}, we show an example sequence for $k=5$ where the samples from the last $5$ time steps are the same as the samples from the first $5$ time steps. In order to learn such sequences, the models must to have the ability to learn signals with temporal delays of length $l$. 
\item [\textbf{Context-Addressed Dependency Task}] In this task, we wish to explore sequences with dynamic temporal dependencies unlike the first two tasks where dependencies were long-range but fixed. To accomplish this, we use the labels of MNIST digits as a form of 'address in time' in sequence generation process. First, a \emph{random sequence} of length $l$ is created as before. In each step $t$ of the next $k$ generations, we determine the digit label of the most recently generated sample, call it $l_{t-1}$, and use this number as an 'address in time' over the \emph{random sequence} and repeat the sample from $l_{t-1}$th time step in $t$. For example, in the third row of Figure \ref{generators}, the last sample is chosen by determining the digit label of the previous sample ($4$ in this case), and repeating the sample from the $4$th position in the \emph{random sequence}. Therefore, the dependencies of the last $k$ steps are determined based on the 'context' of what has been generated already.    
% In this task, we wish to show that our GTMs are able to determine where to direct its attention in the time sequence based on the context of what it has generated already while generating the next step. We want to show that our GTMs can implicitly learn to bind a higher level concept of what it generates to actual time steps and learn data sequences that have non-stationary time delays.
\item [\normalfont \emph{Results}:] In Figure \ref{Task3}, we display samples generated by the \emph{IN}-GTM model after training it with sequences of length $50$. We focus on generation of the last step of the sequence (which is similar in all recall steps). At the last step, the model uses the generated samples from the previous step (red column in Figure \ref{Task3}) by classifying and mapping them to the addresses at the beginning of the sequence to find the samples to recall at the last step. On the right side of the figure, we show where the attention mechanism focuses on at the last step(white boxes) which correspond the addresses indicated in the red column. This extremely complicated relationship is learned purely from sequences that had this property embedded into their structure in a completely unsupervised fashion.

\item [\textbf{One-Shot Recall Task}]
%Training sequences in this task mimic the \emph{Perfect Recall Task} sequences. However, the random samples come from Omniglot dataset instead of MNIST and we are interested in the one-shot generalization of the learned temporal relationships using held-out data. The model is trained to with perfect recall sequences like the first task, but during generation of samples, we give the first $k$ samples as context to the generative model and let it generate the rest of the sequence.   
In this task, we extend the \emph{Perfect Recall Task} to the one-shot learning case in order to determine whether the learned recall ability applies to examples that are never seen during training. In order to do this, we generate training sequences with the same temporal structure as the sequences from the first task with Omniglot dataset while excluding $3$ characters from each alphabet during training. In order to evaluate the one-shot ability of our models, we generate samples by giving our model the first $k$ steps (which are normally recalled at the end of sequences) as a context where each of these samples are from the held out characters of alphabets and let it generate the rest of the sequence. Fourth row of Figure \ref{generators} displays a training sequence from the Omniglot dataset.
\item [\normalfont \emph{Results}:] In Figure \ref{Task4}, we display the context given to our model (from the held out data) and the completed sequence obtained from the generative model. We can see that the recall ability learned from the training set is transferable to new samples that is not seen during training (we qualitatively verified that the imperfections are mostly due to the capacity of the encoder and decoder used by looking at reconstruction of the context, which mimics the samples from last five steps).

\item [\textbf{Stochastic Bouncing Boxes Task}] In this task, we extend the balls bouncing in a box video sequences problem introduced in \cite{NIPS2008_3567} by injecting bi-modal stochasticity at wall collisions. At each collision with the walls, the 'ball' can change shape (solid or holed) with equal probability. In this task we evaluate the ability of our GTMs to model time-homogeneous dynamics with multi-modal transitions and show the natural way to sample from the learned stationary distribution by sampling beyond the length of sequences encountered in training. An example sequence of bouncing balls where the ball collides with the wall can be seen in the last row of Figure \ref{generators}.
\item [\normalfont \emph{Results}:] A sample sequence of $300$ steps is provided in this \href{https://drive.google.com/open?id=0BzjmEb10ZqBMODRXMUtYb0Q2OW8}{link}
The model was trained on sequences of length $30$ and was asked to generate the data for $300$ time steps. By inspecting the attention mechanism during sampling, we see that the model learned that the only dependencies to model are the local dependencies in time. In the video, we can see that the model succeeded in learning the variability in the initial conditions (speed, location of balls), the stationary dynamics of the simple physics as well as the multi-modal transitions of the sprites at collision. 
\end{description}
Appendix \ref{appendix1} provides a further results with step-by-step pseudocode for generating the training sequence for each task.

\subsection*{Generating Coherent Structures From Ego-Centric Viewpoints: MNIST Fields Task}
Generating coherent structures from local views has crucial importance for agents that navigate, plan and act in large spatial environments. For solving problems in such environments, humans can build an internal 'map' of the environment and can imagine random environments that have such spatial coherence even if they have to imagine specific parts of the environments in sequence, possibly through an introspective process.
\begin{figure}[t]
    \includegraphics[width=1\linewidth]{figures/mazes3}
    \label{MnistFields}
    \caption{Left: Training sequence generation process for the \emph{MNIST Fields Task}. First, a random field of MNIST digits is created. Then, an ego-centric viewpoint is moved around the field by taking actions according to a heuristic exploration policy (reach least visited cells in the field) for $L=50$ time steps (there are many revisits). The sequence of ego-centric views (input) and the actions taken (context) are used to train an action-conditional \emph{IN}-GTM. Right: MNIST field generated when the \emph{IN}-GTM is given actions from the training policy. We piece together the whole field from the ego-centric views that the model generates based on the action context. When the model would have revisited a cell by following the given actions, it generates the same exact sample (green overlay) that it generated in the earlier visit to that cell (grey).}
\end{figure}

In the MNIST Fields Task, we train an action-conditional \emph{IN}-GTM, where the inputs are sequences of local views of random fields of MNIST digits during training, along with actions that navigate the environment to obtain those local views as a context (see Figure \ref{MnistFields} for details). In this action-conditional version of the Perfect Recall Task, the model has to learn to do odometry based on the actions and map that odometry to the time sequence to retrieve memories from the past in order to create a coherent structure (because training sequences come from such a coherent structure). Our results in Figure \ref{MnistFields}, show that all of these sub-tasks can be learned in a completely unsupervised fashion though the introspective processes that our model is capable of.


==> results.tex <==
% "Cross-product table"
% Figures showing performance (generated samples, autoencoding, etc.)
% Figures showing KL
% Figures showing learning curves
% References to samples in appendix
\section{Experimental Results}
For all tasks, we present the Kullback-Leibler divergence between the prior and posterior maps, averaged over sequences, measured at each frame in a sequence. We also present the KL divergence at the last frame in a sequence (since this is a predictable frame) as training proceeds. Finally, we show the training loss, the negative Variational Lower Bound, per task. In Appendix \ref{appen:gen_samples}, we present generated samples for most of the tasks. 
For each model, we run 20 replicas with the same hyperparameters. When we perform quantifications for figures, we first average over all 10 example sequences in a mini-batch, then we compute means and standard errors across the replicas for the model type. 

\subsection{Perfect Recall}
In Figure \ref{fig:per_recall_results}, we see results for perfect recall. All models show the effect that the KL-divergence between the prior and posterior becomes reduced at the beginning of the recall phase. However, for the GTMMs and especially the Introspection GTMMs, the reduction is most significant. This implies that the models are predicting the arriving frames based on memory. The effect is more significant for larger sequence lengths.

\begin{figure}
\centering
\includegraphics[width=1\textwidth]{new_figures/learning_curves/PerRec15_summary.pdf}
\includegraphics[width=1\textwidth]{new_figures/learning_curves/PerRec25_summary.pdf}
\includegraphics[width=1\textwidth]{new_figures/learning_curves/PerRec55_summary.pdf}
\caption{\emph{Top Row}: the perfect recall task with $l=10$ and $k=5$. \emph{Left:} The average Kullback-Leibler divergence (KLD) per frame, serving as a measure of prediction error between the prior and posterior. Each of the models learns that there is repetition at frame 10, but the Introspection GTMM exhibits the lowest error. \emph{Middle:} The last frame KLD is also lowest for the Introspection GTMM at convergence. \emph{Right:} The Introspective-GTMM convergences fastest and to the lowest level, but we see that the negative variational lower bound is close for all models.
\emph{Middle Row}: the perfect recall task with $l=20$ and $k=5$. The results are roughly similar.
\emph{Bottom Row}: the perfect recall task with $l=50$ and $k=5$. Over substantially larger time intervals, the models are able to detect regularity in the data sequences.
\label{fig:per_recall_results}}
\end{figure}

\subsection{Parity Recall}
For parity recall, less memory is required than for perfect recall as the details of each image need not be retained; instead, only the parity of each image should be tracked, requiring 5 bits total. All models perform satisfactorily here, as we see in Figure \ref{fig:par_recall_results}, exhibiting KL reductions when the number of possible digit classes drops from 10 to only 1 (the remembered parity digit images). The models are able to contend with long delays equally, suggesting that the primary advantage for GTMMs over VRNNs is in tasks that require the storage of a large number of bits.

\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{new_figures/learning_curves/ParRec15_summary.pdf}
	\includegraphics[width=1\textwidth]{new_figures/learning_curves/ParRec25_summary.pdf}
	\includegraphics[width=1\textwidth]{new_figures/learning_curves/ParRec55_summary.pdf}	
    \caption{\emph{Top Row}: the parity recall task with $l=10$ and $k=5$. The difference between models is minimal here, likely because the memory storage required to solve the task is only $k=5$ bits.
    \emph{Middle Row}: the task with parameters $l=20$ and $k=5$.
    \emph{Bottom Row}: with $l=50$ and $k=5$. Again, all models succeed equally despite the longer delay.    
    \label{fig:par_recall_results}}
\end{figure}

\subsection{One-Shot Recall}
For the one-shot recall task, the GTMMs all outperform the VRNN with the Introspective-GTMM showing significant reductions in KL divergence at the beginning of the recall phase (Figure \ref{fig:omni_recall_results}). This is notable because the memorised images are entirely novel hold-outs from the training set.
Thus, the GTMMs, and in particular the Introspective-GTMM, are able to construct useful latent variable representations for novel stimuli, store them in memory, and use them to predict future events during the recall phase.
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{new_figures/learning_curves/OmniRec25_summary.pdf}
    \caption{The one-shot recall task with experimental parameters $l=20$ and $k=5$. Again, because the task is very similar to perfect recall in structure, the models perform in a comparable rank order, with the Introspective-GTMM showing significant KL reductions when the sequence is predictable from memory.
    \label{fig:omni_recall_results}}
\end{figure}

\subsection{Learning Dynamic Dependencies}
The dynamic dependency task requires the models to learn an algorithmic addressing procedure in which the current image indicates the time point the next image was stored, allowing the memory address storing the latent variables from that time point to be looked up. All of the GTMMs perform considerably better than the VRNN on the task, with the most substantial improvements achieved by the Introspective-GTMM and the DNC-GTMM (Figure \ref{fig:dyn_dep_results}).
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{new_figures/learning_curves/Context25_summary.pdf}
    \caption{Dynamic dependency task with $l=20$ and $k=5$: The DNC-GTMM and the Introspective-GTMM are the best at this complex addressing task.
    \label{fig:dyn_dep_results}}
\end{figure}

\subsection{Similarity-Cued Recall}
Similarity-cued recall plays more strongly to the advantages of memory systems with content-based addressing. The task requires using a cue image to find the images in sequence that followed the cue during the pre-recall exposure phase. To perform this operation, the memory systems with content-based addressing, the NTM, LRU, and DNC, can encode the cue and look up similar feature encodings in memory. As long as there is a mechanism to iterate through the subsequent latent variables, the task can then be easily solved. DNC-GTMM can use its temporal transition links for this task, as described in \citep{graves2016hybrid}. Because it lacks content-based addressing, the Introspective-GTMM does not perform better than the VRNN (Figure \ref{fig:content_results}).
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{new_figures/learning_curves/Content25_summary.pdf}
    \caption{Similarity-cued recall with temporal dependencies of length $l=20$ and $k=5$. The memory models with content-based addressing, i.e., the NTM-, LRU-, and DNC-GTMM, show the most significant KL reductions and lowest task losses.
    \label{fig:content_results}}
\end{figure}

\subsection{Navigation in an MNIST Map}
\begin{figure}
	\centering
	\includegraphics[width=1.\textwidth]{new_figures/learning_curves/mnistMaze25_summary.pdf}
    \caption{MNIST Maze task. The GTMMs with content-based addressing acquire information about the environment and can coherently model it.
    \label{fig:mnist_maze_results}}
\end{figure}
Our next task requires a model to represent the coherent spatial structure of a two-dimensional grid. Since the actions are generated by a random walk process, the structure of this problem is poorly captured by memory addressing mechanisms that are based on time or positional order in a sequence. Instead, models that use content-based addressing can encode the sequence of actions alongside the latent variable representations of the images. When it is necessary to predict what is present at an already visited location, content-based addressing can be used to look up the latent variables based on the action sequence. Since any grid cell can be reached via multiple routes, the models must also capture the invariance that action sequences should be converted into displacements from the origin. The DNC- and LRU-GTMM perform best at this task (Figure \ref{fig:mnist_maze_results}), exhibiting significant KL reductions as more of the environment is explored. In Figure \ref{fig:mnist_maze_overlay}, we also show generation of a sequences in the maze by each model. Only LRU-GTMM and DNC-GTMM consistently generate the same digits when returning to the same positions.

Although the NTM-backed GTMM has content-based addressing, its ability to allocate free locations in memory is generally inferior to the abilities of models using LRUs and DNCs. The LRU- and DNC-based mechanisms can easily store new memories but also can collocate the new memories with decorative meta-information registering on which position on the grid each image is located.  

\begin{figure}
	\centering
	\includegraphics[width=1.\textwidth]{new_figures/MnistMaze/mnMaze_summary}
    \caption{Generation examples in the MNIST Maze. Actions are shown in the top row. In each column of that row, the last five actions at each time point ($t=5, 10, 15, \dots$) are indicated by yellow arrows. The best four models of each type are shown in each row below. The first time a grid cell is visited, the red pixel channel is turned on; the second time, a new image is generated and super-imposed, with the red and green channels turned on (so overlaid image colour is red+green=yellow); the third time, the blue channel is turned on, so the overlaid, generated image is white. We see that the VRNN has inconsistent generations, as the subsequent visits to grid cells produce overlays of different colours that do not share the same shape. The NTM and Introspection models are by comparison better at coherent generation, and the LRU- and DNC-based GTMMs are the best here, so that, for example, the white and yellow digits mask the underlying red digit.
    \label{fig:mnist_maze_overlay}}
\end{figure}

\subsection{Coherence in Realistic Environments}
In Figure \ref{fig:fast_rot_summary}, we see that the VRNN has the lowest variational lower bound. However, in the generative samples, it is clear that the VRNN is also incoherent across time, as it forgets information about paintings on the walls and buildings on the skyline (Figure, \ref{fig:fast_rot_gen}). We argue that the more representative quantification, of more significance than the training loss, is the Kullback-Leibler divergence of the last frame, as well as the KL reduction at the time of the turn. These indicators show that the DNC and Introspection network models are able to predict the redundant frames from memory.

\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{new_figures/learning_curves/FastRot_summary.pdf}
    \caption{Realistic environments task. The VRNN has the lowest variational lower bound, but this measure tells very little of the overall story. Instead, the DNC-GTMM and Introspection-GTMM show significant KL reductions when the sequence is predictable from memory, and this measure translates into good behaviour during generation of samples.
    \label{fig:fast_rot_summary}}
\end{figure}

%\subsection{Sequences involving realistic 3-D environments}
% Might be worth expanding on the difficulty of this problem -- the frames don't align after the rotation, so the model really has to learn some tricky things (perspective, global structure, etc.) in order to produce good samples. 


%\subsection{Control experiments}

%\todo{Adam: just trying out some different orientations for the figures plotted above -- they're basically the same as those generated by Mevlana below, but with different spacing, font sizes, etc}
% \pagebreak
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=6cm 0.5cm 5cm 0.5cm, width=0.5\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_15_5_Model_vRNN_task_0}
% 	\includegraphics[clip, trim=6cm 0.5cm 5cm 0.5cm, width=0.5\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_15_5_Model_Comb_task_0}
% 	\includegraphics[clip, trim=6cm 0.5cm 5cm 0.5cm, width=0.5\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_15_5_Model_IntroD_task_0}
% 	\includegraphics[clip, trim=6cm 0.5cm 5cm 0.5cm, width=0.5\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_15_5_Model_LRU_task_0}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/PerRec/KLLast_MeanNonTracedPerRec_seqLen15_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/KLAll_MeanNonTracedPerRec_seqLen15_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/lowerBound_MeanNonTracedPerRec_seqLen15_5_leg_True.pdf}
%     \caption{Results for \emph{Perfect Recall} task with temporal dependencies of length $l=10$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_25_5_Model_vRNN_task_1}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_25_5_Model_Comb_task_0}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_25_5_Model_IntroD_task_0}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_25_5_Model_LRU_task_0}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/PerRec/KLLast_MeanNonTracedPerRec_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/KLAll_MeanNonTracedPerRec_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/lowerBound_MeanNonTracedPerRec_seqLen25_5_leg_True.pdf}
%     \caption{Results for \emph{Perfect Recall} task with temporal dependencies of length $l=20$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=10.5cm 0.5cm 8.5cm 0.5cm, width=0.7\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_35_5_Model_vRNN_task_0}
% 	\includegraphics[clip, trim=10.5cm 0.5cm 8.5cm 0.5cm, width=0.7\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_35_5_Model_Comb_task_0}
% 	\includegraphics[clip, trim=10.5cm 0.5cm 8.5cm 0.5cm, width=0.7\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_35_5_Model_IntroD_task_0}
% 	\includegraphics[clip, trim=10.5cm 0.5cm 8.5cm 0.5cm, width=0.7\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_35_5_Model_LRU_task_0}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/PerRec/KLLast_MeanNonTracedPerRec_seqLen35_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/KLAll_MeanNonTracedPerRec_seqLen35_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/lowerBound_MeanNonTracedPerRec_seqLen35_5_leg_True.pdf}
%     \caption{Results for \emph{Perfect Recall} task with temporal dependencies of length $l=30$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_55_5_Model_vRNN_task_0}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_55_5_Model_Comb_task_0}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_55_5_Model_IntroD_task_0}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_55_5_Model_LRU_task_0}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/PerRec/KLLast_MeanNonTracedPerRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/KLAll_MeanNonTracedPerRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/lowerBound_MeanNonTracedPerRec_seqLen55_5_leg_True.pdf}
%     \caption{Results for \emph{Perfect Recall} task with temporal dependencies of length $l=50$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_25_5_Model_vRNN_task_4}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_25_5_Model_Comb_task_3}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_25_5_Model_IntroD_task_1}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_25_5_Model_LRU_task_4}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/Cntxt/KLLast_MeanNonTracedCntxt_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/Cntxt/KLAll_MeanNonTracedCntxt_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/Cntxt/lowerBound_MeanNonTracedCntxt_seqLen25_5_leg_True.pdf}
%     \caption{Results for \emph{One-shot Recall} task with temporal dependencies of length $l=20$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_55_5_Model_vRNN_task_1}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_55_5_Model_Comb_task_4}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_55_5_Model_IntroD_task_0}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/Cntxt/samples/ex_Task_Cntxt_SeqLen_55_5_Model_LRU_task_4}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/Cntxt/KLLast_MeanNonTracedCntxt_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/Cntxt/KLAll_MeanNonTracedCntxt_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/Cntxt/lowerBound_MeanNonTracedCntxt_seqLen55_5_leg_True.pdf}
%     \caption{Results for \emph{Learning Dynamic Dependencies} task with temporal dependencies of length $l=50$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_25_5_Model_vRNN_task_4}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_25_5_Model_Comb_task_3}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_25_5_Model_Intro_task_4}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_25_5_Model_LRU_task_4}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/OmnRec/KLLast_MeanNonTracedOmnRec_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/OmnRec/KLAll_MeanNonTracedOmnRec_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/OmnRec/lowerBound_MeanNonTracedOmnRec_seqLen25_5_leg_True.pdf}
%     \caption{Results for \emph{One-shot Recall} task with temporal dependencies of length $l=20$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_55_5_Model_vRNN_task_1}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_55_5_Model_Comb_task_4}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_55_5_Model_Intro_task_1}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/OmnRec/samples/ex_Task_OmnRec_SeqLen_55_5_Model_LRU_task_4}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/OmnRec/KLLast_MeanNonTracedOmnRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/OmnRec/KLAll_MeanNonTracedOmnRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/OmnRec/lowerBound_MeanNonTracedOmnRec_seqLen55_5_leg_True.pdf}
%     \caption{Results for \emph{One-Shot Recall} task with temporal dependencies of length $l=50$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_25_5_Model_vRNN_task_4}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_25_5_Model_Comb_task_3}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_25_5_Model_IntroD_task_4}
% 	\includegraphics[clip, trim=7.5cm 0.5cm 6cm 0.5cm, width=0.6\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_25_5_Model_LRU_task_4}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/ParRec/KLLast_MeanNonTracedParRec_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/ParRec/KLAll_MeanNonTracedParRec_seqLen25_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/ParRec/lowerBound_MeanNonTracedParRec_seqLen25_5_leg_True.pdf}
%     \caption{Results for \emph{Parity Recall} task with temporal dependencies of length $l=20$ ($k=5$).}
% \end{figure}

% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_55_5_Model_vRNN_task_1}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_55_5_Model_Comb_task_4}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_55_5_Model_IntroD_task_1}
% 	\includegraphics[clip, trim=17cm 0.5cm 13cm 0.5cm, width=0.9\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/ParRec/samples/ex_Task_ParRec_SeqLen_55_5_Model_LRU_task_4}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/ParRec/KLLast_MeanNonTracedParRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/ParRec/KLAll_MeanNonTracedParRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/ParRec/lowerBound_MeanNonTracedParRec_seqLen55_5_leg_True.pdf}
%     \caption{Results for \emph{Parity Recall} task with temporal dependencies of length $l=50$ ($k=5$).}
% \end{figure}
% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=33.5cm 0.5cm 26cm 0.5cm, width=0.9\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_105_5_Model_vRNN_task_0}
% 	\includegraphics[clip, trim=33.5cm 0.5cm 26cm 0.5cm, width=0.9\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_105_5_Model_Comb_task_0}
% 	\includegraphics[clip, trim=33.5cm 0.5cm 26cm 0.5cm, width=0.9\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_105_5_Model_IntroD_task_0}
% 	\includegraphics[clip, trim=33.5cm 0.5cm 26cm 0.5cm, width=0.9\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/PerRec/samples/ex_Task_PerRec_SeqLen_105_5_Model_LRU_task_0}
% 	\includegraphics[clip, trim=3cm 2cm 3cm 2cm, width=0.9\textwidth]{figures/results/PerRec/KLLast_MeanNonTracedPerRec_seqLen105_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=0.45\textwidth]{figures/results/PerRec/KLAll_MeanNonTracedPerRec_seqLen105_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=0.45\textwidth]{figures/results/PerRec/lowerBound_MeanNonTracedPerRec_seqLen105_5_leg_True.pdf}
%     \caption{Results for \emph{Perfect Recall} task with temporal dependencies of length $l=100$ ($k=5$).}
% \end{figure}


% \begin{figure}[H]
% 	\centering
% 	\includegraphics[clip, trim=0cm 0.5cm 0cm 0.5cm, width=0.8\textwidth, cfbox=yellow!98!black 1pt 1pt]{figures/results/PerRec/samples/105VRNN}
% 	\includegraphics[clip, trim=0cm 0.5cm 0cm 0.5cm, width=0.8\textwidth, cfbox=blue!70 1pt 1pt]{figures/results/PerRec/samples/105Comb}
% 	\includegraphics[clip, trim=0cm 0.5cm 0cm 0.5cm, width=0.8\textwidth, cfbox=green!70!black 1pt 1pt]{figures/results/PerRec/samples/105Intro}
% 	\includegraphics[clip, trim=0cm 0.5cm 0cm 0.5cm, width=0.8\textwidth, cfbox=red!70!black 1pt 1pt]{figures/results/PerRec/samples/105LRU}
% 	\includegraphics[clip, trim=3cm 0cm 3cm 2cm, width=0.9\textwidth]{figures/results/PerRec/KLLast_MeanNonTracedPerRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/KLAll_MeanNonTracedPerRec_seqLen55_5_leg_True.pdf}
%     \includegraphics[clip, trim=0cm 0cm 0cm 2cm, width=0.45\textwidth]{figures/results/PerRec/lowerBound_MeanNonTracedPerRec_seqLen55_5_leg_True.pdf}
%     \caption{Results for \emph{Perfect Recall} task with temporal dependencies of length $l=100$ ($k=5$).}
% \end{figure}

==> resultsIntro.tex <==
\section{Results}
\label{sect:results}
% "Cross-product table"
% Figures showing performance (generated samples, autoencoding, etc.)
% Figures showing KL
% Figures showing learning curves
% References to samples in appendix



%\subsubsection{Learning}




==> someOldContentForResults.tex <==

\section{Results}
\subsubsection{Perfect recall}
\item [\normalfont \emph{Results and comparison}:] % Performance in this task is assessed in two ways. 
% First, we measure the $D_{KL}$ of the latent code across the training sequence; if the network makes use of previously encoded information from already seen samples, then the amount of information the encoder needs to transmit is reduced, which in turn reduces the $D_{KL}$. 
% Since the only reliable information that can be re-used is from the first $k$ samples, a reduction in the $D_{KL}$ for the final $k$ samples is indicative of proper encoding, long-term storage, and retrieval of information in memory. 
% Second, we generate samples from the generative model component of the network to see if generated sequences are consistent with the constraints set out by the task -- namely, that the first $k$ samples are identical to the final $k$ samples in the generated sequence. 

In Figure \ref{Task1}, we present samples from an \emph{IN}-GTM that was trained on such sequences of length $L = 50$ (see Appendix \ref{AppendResults} for $L = 100$). We observe that the last $k=5$ steps were generated based on the past generations through perfect recall by focusing on the relevant parts of the sequence with the attention mechanism (see attention weights at top of Figure \ref{Task1}). 




In Figure \ref{ResKLVRNN}(left), we compare \emph{IN}-GTMs against VRNN variants in this task by displaying the evolution of the KL divergence term for the last recall step during training. This term is proportional to the number of bits of information required to reconstruct the sample at that step using the previous samples. If the temporal relationship is learned and the model can do a perfect recall using the past, this value would be very low ($<5$ nats) compared to the number of bits required for a random MNIST digit ($~20$ nats). 

We observe that for \emph{IN}-GTMs, the KL divergences go to $~3$ nats (accomplishes perfect recall) in $<10$k training iterations in a stable way when the temporal delays for recall are around $L = 50$ and $L = 100$ time steps. On the other hand, we present results from VRNN variants only for $L = \{3, 5, 10\}$ sequences. Throughout our experiments, these models were \textbf{not} able to learn the perfect recall relationship with temporal delays of length $>10$. Even in the case of $L = \{5, 10\}$, majority of our experiments did not succeed and there was a large variation in the number of steps of training it took for these models to learn the temporal relationship, whereas \emph{IN}-GTMs have been robust throughout. E.g. one of the two successful models for $L = 3$ in Figure \ref{ResKLVRNN} learns in $<10$k iterations while the other takes $>100$k iterations. 

\subsubsection{Parity Recall}
In Figure \ref{Task2}, we display samples generated by the \emph{IN}-GTM model after training it with sequences of length $50$. We see that the model generates random $0$s and $1$s in the last five steps based on the parity of the first five samples in the sequence (Refer to appendix for class transition matrices between the first and last five steps of the sequences and the full algorithm for the generative process for this task).

%Similar to the first task, we first create a \emph{random sequence} of MNIST digits for $l$ time steps. In this task, instead of repeating past samples for the next $k$ time steps, we take an arbitrary function over the MNIST classes (evenness/oddness) of the samples from the past and generate random $1$s and $0$s corresponding to evenness of the first $k$ samples from the beginning of the \emph{random sequence}. In the first row of figure \ref{generators}, we show an example sequence for $k=5$ where the samples from the last $5$ time steps are the same as the samples from the first $5$ time steps

%. In the first row of figure \ref{generators}, we show an example sequence for $k=5$ where the samples from the last $5$ time steps are the same as the samples from the first $5$ time steps. In order to learn such sequences, the models must to have the ability to learn signals with temporal delays of length $l$. 

\subsubsection{Semantic Dependency Task}
In Figure \ref{Task3}, we display samples generated by the \emph{IN}-GTM model after training it with sequences of length $50$. We focus on generation of the last step of the sequence (which is similar in all recall steps). At the last step, the model uses the generated samples from the previous step (red column in Figure \ref{Task3}) by classifying and mapping them to the addresses at the beginning of the sequence to find the samples to recall at the last step. On the right side of the figure, we show where the attention mechanism focuses on at the last step(white boxes) which correspond the addresses indicated in the red column. This extremely complicated relationship is learned purely from sequences that had this property embedded into their structure in a completely unsupervised fashion.

\subsubsection{One-Shot Recall Task}
In Figure \ref{Task4}, we display the context given to our model (from the held out data) and the completed sequence obtained from the generative model. We can see that the recall ability learned from the training set is transferable to new samples that is not seen during training (we qualitatively verified that the imperfections are mostly due to the capacity of the encoder and decoder used by looking at reconstruction of the context, which mimics the samples from last five steps).

% \item [\textbf{Stochastic Bouncing Boxes Task}] In this task, we extend the balls bouncing in a box video sequences problem introduced in \cite{NIPS2008_3567} by injecting bi-modal stochasticity at wall collisions. At each collision with the walls, the 'ball' can change shape (solid or holed) with equal probability. In this task we evaluate the ability of our GTMs to model time-homogeneous dynamics with multi-modal transitions and show the natural way to sample from the learned stationary distribution by sampling beyond the length of sequences encountered in training. An example sequence of bouncing balls where the ball collides with the wall can be seen in the last row of Figure \ref{generators}.
% \item [\normalfont \emph{Results}:] A sample sequence of $300$ steps is provided in this \href{https://drive.google.com/open?id=0BzjmEb10ZqBMODRXMUtYb0Q2OW8}{link}
% The model was trained on sequences of length $30$ and was asked to generate the data for $300$ time steps. By inspecting the attention mechanism during sampling, we see that the model learned that the only dependencies to model are the local dependencies in time. In the video, we can see that the model succeeded in learning the variability in the initial conditions (speed, location of balls), the stationary dynamics of the simple physics as well as the multi-modal transitions of the sprites at collision. 
% \end{description}
% Appendix \ref{appendix1} provides a further results with step-by-step pseudocode for generating the training sequence for each task.

\subsubsection{MNIST Map Task}
Our results in Figure \ref{MnistFields}, show that all of these sub-tasks can be learned in a completely unsupervised fashion though the introspective processes that our model is capable of.

\subsubsection{In-place rotations in a realistic 3-D environment}
\subsubsection{Loop closures in a realistic 3-D environment}


\subsection{Evaluation Methodology}
We evaluate the \emph{Introspection Network} based GTMs (\emph{IN}-GTM) by comparing them against VRNNs \cite{chung2015recurrent} described in section \ref{sect:GTM} on five tasks that expose different aspects of temporal modelling  that a GTM should satisfy. For each task, we created temporal sequences based on benchmark datasets, e.g., MNIST\cite{MnistCitation}, Omniglot\cite{omniglotCitation} and Bouncing Balls in a Box\cite{NIPS2008_3567}. A successful GTM should perform well in all tasks and generate compelling samples that mimic the temporal relationships embedded in the sequences. These tasks are:
\begin{description}[leftmargin=*,topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item[Perfect Recall Task.] Tests the ability to preserve information without interference across long time-scales efficiently.
\item[Even-Odd Transition Task.] Tests the ability to learn arbitrary and complex relationships between time steps.
\item[Context-Addressed Dependency Task] tests the ability to condition on specific places in the time sequence based on the context of what has been generated already while generating the next step.
\item[One-Shot Recall Task.] Tests the ability to do one-shot generalisation, i.e. successfully apply learned temporal relationships to examples that are never seen during training.
\item[Stochastic Bouncing Balls Task.] Tests the ability to model the stationary distribution of the sequences where there are inherent multimodalities involved.
\end{description} 
%
% in their temporal relationships and train our GTMs to discover these relationships from training sequences.
%If the models are able to learn the underlying distributions of the sequences properly, they should be able to generate sample sequences that mimic the sequences from training.

%\subsubsection{Learning}
We train each model with stochastic gradient descent on the variational lower bounds \eqref{eq:FE} using the Adam optimizer [12], with a learning rate of 0.001. We experimented with different latent variable sizes $K=\{10, 20, 50\}$ and used a minibatch size of $10$ for \emph{IN}-GTMs and $10$ or $24$ for VRNN variants. For both \emph{IN}-GTMs and VRNNs, the functions that parameterize the inference and the generative models are $3$-layer convolutional and deconvolutional residual networks \cite{he2015deep}, respectively. In addition, we experimented with much higher capacity networks for VRNNs with larger MLPs and LSTM hidden units (we discuss the relevant two cases $h=200$ and $h=300$ in our results) compared to \emph{IN}-GTMs. In \emph{IN}-GTMs, we always use an episodic memory of maximum size equal to the length of the training sequences minus one. This length can be in the order of hundreds (see Appendix \ref{AppendResults} for results with $100$ step sequences) without a heavy memory burden as long as the latent space is compact. In comparison, in the small number of experiments where VRNN variants had some success modeling temporal relationships of length $<15$, they had to use more memory overall than \emph{IN}-GTMs that was successful at modeling relationships of length $>50$ .

Initialization of the attention mechanism however is an important factor during optimization since, as the memory size increases, there is a linearly increasing interference in the temporal signal which reduces the signal-to-noise ratio. In the \emph{Introspection Network} architecture, we allocate \emph{parallel} read heads that are initialized with biases that allow for \emph{local} search of the specific parts of the episodic memory in order to increase temporal exploration and speed up optimization. For a temporal sequence of $100$ steps, having $5$ \emph{parallel} heads which have relatively high biases for sub-sequences $[1, 20], [21, 40], [41, 60], [61, 80], [81, 100]$ respectively, can speed up learning tremendously compared to initializing all biases uniformly. During our experiments, we have seen that even with a sharp initialization of these biases, the read heads eventually move to locations with low initial biases during training if they have to in order to model the temporal relationships.\todo{make this fit into text}

==> temporary_visual_architectures.tex <==
MNIST Problems & Omniglot


The posterior map CNN consisted of two processing blocks. The input to each block was sent through four dimension-preserving parallel convolution streams using 8 kernels of size 1x1, 3x3, 5x5, and 7x7, respectively. The outputs from these convolutions were passed through a batch-normalisation layer [cite here], and then through a rectified linear layer, concatenated, and convolved again with a down-sampling kernel of size 3x3, which halved the dimension size the input. This was then passed through a batch-normalisation layer, followed by a rectified linear layer, except for the block before the latent variable. The entire CNN consisted of two of these blocks positioned serially. Therefore, input images of size 32x32 were convolved to 32 feature-maps of size 8x8.

deconv: 
For observation maps, we use the exact same sequence of operations, except that each convolution is replaced with a deconvolution module.

Labyrinth
\todo{Labyrinth visual module description}


The  posterior  map  -- that is, the mapping from inputs $x_t$ to latents $z_t$ -- was implemented as a convolutional neural network (CNN). The CNN consisted of two ``blocks," placed serially. The first block was fed a 3x32x32 color image, or 1x32x32 black-and-white image as input. This input was passed to four parallel dimension-preserving convolutional streams, which convolved the input using 8 kernels of size 1x1, 3x3, 5x5, and 7x7, respectively. The outputs from the parallel streams were passed through a batch-normalization layer, and a rectified-linear layer, before being concatenated to a total of 32 feature-maps. These 32 feature-maps served as the input to a dimension-halving convolution using a kernel of size 3x3, which was followed by a batch normalization layer and a rectified linear layer. Thus, this first processing block functioned to take in an 32x32 image as input and return 32 feature-maps of size 16x16. A second block followed from the first. This block was identical to the first, except for two differences: there was no batch normalization and rectified layer after the final convolution, and the final number of kernels was 64.

These processing blocks, then, processed a 32x32 image into 64 feature maps of size 8x8. As mentioned, the posterior map infers latents $z_t$ from inputs $x_t$. To implement this mapping, we used the first 32 feature maps as $\mu$ values and the last 32 feature maps as $\log \sigma$ values, which, together with an auxilliary noise variable $\epsilon$, computed $z_t = \mu_t + \sigma_t \epsilon_t$, thus completing the posterior map. The observation map -- the mapping from latents $z_t$ to reconstructions $\hat{x}_t$ -- was identical to the posterior map, except convolution operations were replaced with deconvolution operations. 
